LAMD: Context-driven Android Malware Detection and Classification with LLMs

The rapid growth of mobile applications has escalated Android malware threats. Although there are numerous detection methods, they often struggle with evolving attacks, dataset biases, and limited explainability. Large Language Models (LLMs) offer a promising alternative with their zero-shot inference and reasoning capabilities. However, applying LLMs to Android malware detection presents two key challenges: (1)the extensive support code in Android applications, often spanning thousands of classes, exceeds LLMs' context limits and obscures malicious behavior within benign functionality; (2)the structural complexity and interdependencies of Android applications surpass LLMs' sequence-based reasoning, fragmenting code analysis and hindering malicious intent inference. To address these challenges, we propose LAMD, a practical context-driven framework to enable LLM-based Android malware detection. LAMD integrates key context extraction to isolate security-critical code regions and construct program structures, then applies tier-wise code reasoning to analyze application behavior progressively, from low-level instructions to high-level semantics, providing final prediction and explanation. A well-designed factual consistency verification mechanism is equipped to mitigate LLM hallucinations from the first tier. Evaluation in real-world settings demonstrates LAMD's effectiveness over conventional detectors, establishing a feasible basis for LLM-driven malware analysis in dynamic threat landscapes.

==> Algorithm/Invariant_training.tex <==
\begin{algorithm}[htb]
\caption{Algorithm of Invariant Training}
\label{alg1}
    \begin{algorithmic}[1]
    \REQUIRE ~training dataset containing $|\mathcal{E}|$ environments $\mathcal{D}_{tr}$ and each sample $x$ has a binary classification label $y_{c}, c \in [0, 1]$ and an environment label $y_e, e \in \mathcal{E}$, batch size $|\mathcal{B}|$, predefined number of epochs for stage 1 training $N$, hyperparameters $\alpha$ and $\beta$ for loss weighting, model $f$ with encoder network $\phi$ and predictor $h$. 
    \ENSURE 
    \STATE \textbf{Stage 1: Discriminative Information Amplification}
    \FOR{$\text{epoch} = 1$ to $N$}
        \FOR{$i = 1, \ldots, |\mathcal{B}|$}
            \FOR{$e \in \mathcal{E}$}
            \STATE select mini-batch of samples ${x_i^{e}} \subseteq \mathcal{B}$ \\
            \STATE calculate classification loss $\mathcal{L}^{e}_{CLS}$\\
            \STATE calculate multi-proxy contrastive loss $\mathcal{L}^{e}_{MPC}$ \\
            \ENDFOR
        \STATE obtain loss for empirical risk minimization $\mathcal{L}_{ERM} = \frac{1}{|\mathcal{E}|} \sum_{e \in \mathcal{E}} \mathcal{L}^{e}_{CLS} + \alpha \cdot \mathcal{L}^{e}_{MPC}$
        \STATE update $f$ by backpropagating $\mathcal{L}_{ERM}$
        \ENDFOR
    \ENDFOR
    \STATE \textbf{Stage 2: Unstable Information Suppression}
    \STATE Reset optimizer parameters
    \STATE Continue with model parameters from Stage 1\\
    \FOR{$\text{epoch} = N+1$ to $\text{TotalEpochs}$}
        \FOR{$i = 1, \ldots, |\mathcal{B}|$}
            \STATE get representations $\mathbf{z}_i \gets \phi(x_i)$
            \FOR{$e \in \mathcal{E}$}
            \STATE select mini-batch of representations ${\mathbf{z}_i^{e}} \subseteq \mathbf{z}_i$ \\
            \STATE initialize dummy classifier $\{s_{e} = 1.0\}$ \\
            \STATE calculate invariant gradient alignment loss $\mathcal{L}^e_{IGA}$ \\
            \ENDFOR
            \STATE get predicted labels $\tilde{y}_c \gets f(\mathbf{z}_i)$ \\
            \STATE obtain classification loss $\frac{1}{|\mathcal{E}|}\sum_{e \in \mathcal{E}}\mathcal{L}^e_{IGA}$ \\
            \STATE $\mathbf{p}_{c} \gets \text{mean}(\mathbf{z}_c),c \in [0, 1]$ \\
            \STATE obtain multi-proxy contrastive loss $\mathcal{L}_{MPC}$ \\
            \STATE $\mathcal{L}_{IRM} \gets \mathcal{L}_{CLS} + \alpha \cdot \mathcal{L}_{MPC} + \beta \cdot \frac{1}{|\mathcal{E}|}\sum_{e \in \mathcal{E}}\mathcal{L}^e_{IGA}$ \\
            \STATE update $f$ by backpropagating $\mathcal{L}_{IRM}$
        \ENDFOR
    \ENDFOR
    \end{algorithmic}
\end{algorithm}

==> History/Conclusion.tex <==
\section{Conclusion}
Android malware detectors face performance degradation due to distribution shifts from malware evolution. Our findings reveal invariant patterns among malware samples with similar intents, creating a stable feature space over time. However, ERM-based detectors, limited by i.i.d. assumptions, struggle to capture these invariances due to disrupted malware release sequences. To address this, we propose a temporal invariant training framework that organizes samples into temporally ordered subsets, exposing evolutionary patterns to help arbitrary detectors capture cross-subset invariances and enhance performance on temporally distant samples. Our framework combines multi-proxy contrastive learning with invariant gradient alignment, allowing the model to focus on stable, discriminative features within complex malware distributions. Systematic evaluations across feature spaces and drift scenarios show that this approach significantly enhances robustness, enabling the model to learn enduring, discriminative patterns over time.
% Android malware detectors suffer performance degradation due to distribution shifts from malware evolution. Our findings reveal invariant patterns among malware samples with similar intents, forming a stable and effective feature space over time. However, ERM-based detectors, constrained by i.i.d. assumptions, struggle to capture these invariances due to the disrupted sequence of malware releases. To address this, we propose a temporal invariant training framework for malware detection, organizing samples into temporally ordered subsets that expose evolutionary patterns during training, enabling the model to capture cross-subset invariances and improve performance on temporally distant test samples. Our framework integrates multi-proxy contrastive learning with invariant gradient alignment to model complex malware distributions, allowing the detector to focus on stable, discriminative features. Systematic evaluations across feature spaces and drift scenarios demonstrate that this approach significantly enhances robustness, enabling the model to learn enduring, discriminative patterns over time.

==> History/Discussion.tex <==
\section{Discussion}
\subsection{Influence of Malware Ground Truth}
Malware labels are determined based on the decisions of multiple security engines, which often disagree on whether a given sample is malware or not. Researchers typically establish a threshold to classify samples, balancing sensitivity and specificity. Lower thresholds tend to include more borderline or grey software that resembles benign applications, thereby blurring classification boundaries. In this paper, we select a lower threshold, vt = 4, to evaluate the performance of our approach in this challenging scenario.
% In most studies, malware labels are determined based on the decisions of multiple security engines, which often disagree on whether a given sample is malicious. Researchers typically set a threshold based on experience to determine basic facts about malware, leading to inconsistencies. A lower threshold includes more grayware, blurring decision boundaries as these samples resemble benign software. A higher threshold reduces malicious samples, potentially missing threats due to modern obfuscation techniques. In this section, we evaluate the impact of thresholds 4 and 12 on performance, using 2014 samples as the training set and the table~\ref{tab:ground_truth} shows the AUT(F1,12m) for subsequent years.


\input{Table/Regularization}
% \input{Table/Ground_truth}


\subsection{Comparison to the Regularization Method}
ERM-trained models often overfit to unstable features, limiting test set generalization~\cite{regularization}. Regularization methods, such as early stopping, $\ell$2 regularization, and dropout, help mitigate this by constraining model parameters~\cite{regularization_understanding}. While both regularization and invariant learning improve generalization, invariant learning specifically targets stable features across drift scenarios. We compare these regularization methods with our invariant learning framework during the whole test phase (Table~\ref{tab: regularization}). For reference, DeepDrebin (ERM) includes no regularization, while DeepDrebin~\cite{Grossedeepdrebin} employs dropout with a hyperparameter of 0.2. Results show that adding regularization improves performance under significant drift, with dropout performing best, while early stopping and $\ell$2 leads to poor performance as the model has not yet learnt the best feature representation. Invariant training consistently outperforms, demonstrating its ability to capture highly discriminative, stable features that sustain performance over distant distributions.

\subsection{Application Scope of Invariant Learning}
Invariant learning enhances a model’s generalization to unseen distributions, but keeping stable to all possible shifts is unrealistic. With significant distribution changes, its effectiveness diminishes, and current research indicates that addressing concept drift typically requires costly model updates, including data labeling, retraining, and redeployment. Additionally, pseudo-label noise from automated labeling can further degrade performance~\cite{labelless}. The true value of a robust malware detector lies in sustaining reliable performance under gradual drifts, extending its lifespan before retraining and reducing the cost of selective updates.
% Invariant learning improves the ability of a model to generalize to unseen distributions that may be encountered in the future. However, it is unrealistic to expect the model to adapt perfectly to all possible distributions. When significant distribution changes occur, the ability of invariant learning is weakened. Current research suggests that a complete solution to concept drift is primarily model updating, which entails significant costs, including the costs of labeling new data, retraining, and deployment. Additionally, the impact of noise from pseudo-labels used in automated labeling techniques cannot be ignored~\cite{labelless}. Therefore, the value of a robust malware detector lies in its ability to deliver reliable performance amid gentle drifts. This attribute extends the lifespan of the model before necessitating retraining and ensures that only truly significant samples are annotated and incorporated in updates, ultimately lowering the costs associated with deploying malware detectors.


==> History/Experiment.tex <==
\section{Evaluation}
In this section, we comprehensively evaluate our proposed method's effectiveness in enhancing the drift robustness of Android malware detectors across different feature spaces. Additionally, we examine the specific contributions of each component within the invariant learning framework to the overall robustness improvement. Specifically, our evaluation aims to address the following research questions:
\begin{description}
    \item[RQ1.] Can our method mitigate the aging of detectors based on different feature spaces over time?
    \item[RQ2.] Can our method help the detector to be stable in different drift scenarios?
    \item[RQ3.] Does our method effectively learn the invariant features of applications?
\end{description}
To avoid randomness in the experiments, we chose 1, 42, and 2024 as random seeds to train the model and averaged the test results, respectively. All experiments were performed on RTX A6000. The dataset and code for the experiment will be made publicly available upon acceptance of the paper


\subsection{Evaluation Settings}
\subsubsection{Dataset}
To evaluate the effectiveness of our approach in the context of long-term malware evolution, we select Android APKs from the Androzoo\footnote{https://androzoo.uni.lu} platform, a comprehensive repository aggregating malicious samples from sources like Google Play, PlayDrone, VirusShare, and AppChina. The dataset spans 2014 to 2023, covering ten years of benign and malicious samples. Each sample was analyzed using VirusTotal\footnote{https://www.virustotal.com} and classified as malicious if flagged by more than four vendors. To track malware family evolution, we use Euphony~\cite{euphony} to extract family labels. The dataset includes 251,394 benign and 46,724 malicious applications across 639 families. We adhere to the methodology proposed by TESSERACT~\cite{tesseract} to eliminate potential temporal and spatial biases. The training set covers the year 2014 and the test set the remaining 9 years, from 2015 to 2021. Additionally, the training set is further split into proper training (80\%) and validation (20\%) across all the experimental settings.

%For each evaluation scenario, the samples involved in the training phase are divided into a training set and a validation set in the ratio of 80\% and 20\%.


\subsubsection{Candidate Detectors}
In Android malware detection, an APK file serves as input, containing the codebase (e.g., .dex files) and configuration files (e.g., manifest.xml), which offer behavioral insights such as API calls and permissions. These features are often represented as strings or graphs. To evaluate our invariant training framework, we selected commonly used detectors representing different feature spaces:
\begin{itemize}
    \item Drebin~\cite{Arpdrebin} is a malware detector using binary feature vectors from nine data types (e.g., hardware, API calls, permissions) for linear classification. To align with our framework's focus on neural network architectures, we include its deep learning variant, DeepDrebin~\cite{Grossedeepdrebin}, which uses the same feature space but employs a three-layer deep neural network (DNN) for feature extraction and classification.
    \item Malscan~\cite{malscan} adopts a graph-based feature space, extracting sensitive API calls from APKs and combining four centrality measures (degree, Katz, proximity, and harmonic wave centralities) as features. We concatenate these features according to the optimal method detailed in the paper for detection tasks.
    \item BERTroid~\cite{bertroid} leverages Android application permission strings, encoding them into dense representations with a BERT-based pre-trained model that captures contextual relationships among permissions. For this study, we use the pooled BERT output as the feature representation for malware detection.
    
\end{itemize}
To ensure a fair evaluation of our framework across different feature spaces, we apply two linear layers as the classifier to each of the above feature representations, with the final output layer configured for binary classification.

\subsubsection{Baseline}
To evaluate the robustness of our proposed scheme across various feature spaces, we compare it with two non-linear baseline models: (1) APIGraph~\cite{apigraph}, which enhances robustness using API-based features, and (2) Guided Retraining~\cite{guide_retraining}, which improves detector performance across multiple feature spaces. Additionally, we include T-stability, a feature stability method tailored for linear classifiers in the Drebin~\cite{Arpdrebin} feature space, to highlight the advantages of our non-linear approach. Details of each baseline are as follows:

\begin{itemize}
    \item APIGraph~\cite{apigraph}: This approach clusters APIs, exceptions, and permissions based on semantic similarities from official documentation, creating an API semantic relationship graph. Similar APIs are represented by a clustered index, forming a stable feature space. From the original method, we derive 2,000 clusters, replacing all features within the same cluster with the corresponding index. 
    \item Guided Retraining~\cite{guide_retraining}: This framework improves malware detection by re-partitioning and retraining on challenging samples. Samples are categorized using the base model’s confusion matrix (TN, TP, FN, FP), and supervised contrastive learning extracts group-specific feature representations, enabling separate processing of easy and difficult samples during inference for better accuracy.
    \item T-stability~\cite{svm_ce}: This work introduces t-stability, a metric for SVM models with the Drebin feature space, measuring feature instability via the slope of expected values over time. Then, the above unstable features are constrained to enhance robustness.
\end{itemize}
As APIGraph and T-stability are tailored to specific feature spaces—APIGraph focusing on API call methods and T-stability on manually selected Drebin features~\cite{Arpdrebin}—we use each scheme’s applicable feature space for experiments.



\subsubsection{Metrics}
In the following experiments, we employe static and dynamic evaluation metrics to compare the performance of different approaches. For static evaluation, due to class imbalance in the Android application dataset, we use the macro-F1 score to assess model performance on a fixed-time test set, as it provides a balanced measure of precision and recall.
% Additionally, since the primary goal of the detector is to identify as much malware as possible to minimize security risks, the false negative rate (FNR) is also used as a key metric, with the positive class representing malware. Ideally, a robust detector should maintain a high F1 score and a low FNR under drift, effectively reducing missed detections while keeping the false positive rate reasonable to ensure the detector's usability.

For dynamic evaluation metric, we calculate the Area Under Time (AUT), a metric proposed by TESSERACT \cite{tesseract}, which measures the area under the performance curve as it changes over time. The formula for AUT is as follows:
\begin{equation}
\operatorname{AUT}(m, N)=\frac{1}{N-1} \sum_{t=1}^{N-1}\left(\frac{m(x_t+1)+m(x_t)}{2}\right),
\end{equation}
where $ m$ denotes the performance metric. Here, we select the F1-score as the instance of $m$. $m(x_t)$ denotes the performance metric at time $t$ and $N$ is the number of time slots during the testing phase, with each slot representing a month. AUT values range from $[0, 1]$, where a classifier that performs perfectly would maintain an AUT of 1 throughout all testing time windows. 

\input{Table/RQ1}

\begin{figure}[ht]
    \centering
    % First subfigure
    \begin{subfigure}{0.16\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{Figure/Drebin_rq1.pdf}
        \caption{}
        \label{fig:sub1}
    \end{subfigure}%
    % \hspace{0.01\textwidth} % Adjust this spacing to make the figures more compact
    \hfill
    % Second subfigure
    \begin{subfigure}{0.16\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{Figure/malscan_rq1.pdf}
        \caption{}
        \label{fig:sub2}
    \end{subfigure}%
    % \hspace{0.01\textwidth} % Adjust this spacing to make the figures more compact
    \hfill
    % Third subfigure
    \begin{subfigure}{0.16\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{Figure/bertroid_rq1.pdf}
        \caption{}
        \label{fig:sub3}
    \end{subfigure}
    \caption{Monthly performance of DeepDrebin (a), Malscan (b) and BERTroid (c) feature spaces for the first test year after deployment (2015), with all models initially trained on 2014 samples. \textit{Retrained} indicates detectors updated monthly by incorporating that month's labeled test samples into the original training set.}
    \label{fig:rq1}
    \hfill
\end{figure}

\vspace{-0.5cm}

\subsection{Enhance Different Feature Space (RQ1)}
\label{rq1}
This section evaluates the temporal invariant learning framework (TIF) for mitigating detector degradation across feature spaces. The classifier is trained on 2014 samples and tested monthly from 2015 to 2023, with annual results shown in Table~\ref{tab:rq1}. To optimize short-term performance, we use monthly partitioning, with segmentation granularity discussed in Section~\ref{env seg}. Given that T-stability~\cite{svm_ce} is designed for the Drebin detector, we compare both the original Drebin~\cite{Arpdrebin} and its T-stability variant. APIGraph~\cite{apigraph} supports Drebin and DeepDrebin but is incompatible with BERTroid~\cite{bertroid} and Malscan~\cite{malscan}, while GuideRetraining~\cite{guide_retraining} applies to all detectors. We compare our proposed approach with the baseline model to obtain an absolute performance evaluation. Once deployed, frequently switching between different methods is impractical, even if the model doesn't always yield the best results. Nevertheless, our findings show that, even compared to the best yearly performance of other methods, our approach consistently outperforms them in the long term.

As drift increases over test years, AUT declines for all methods, but TIF maintains a lead, achieving up to an 8\% improvement in the first year. This aligns with real-world scenarios where detectors are retrained annually~\cite{apigraph}. Figure~\ref{fig:rq1} shows 2015 monthly performance, with the grey dashed line marking the upper performance bound. The grey dashed line represents the upper bound of performance for each month. For each month $n$, we split the samples into training and validation sets, label samples from months 1 through $n$ to simulate expert-labelled data, add these to the original training set, and retrain the detector for upper-bound performance evaluation. Without additional labels, TIF approaches this bound, demonstrating robust monthly gains. While AUT gains may diminish over time, this is manageable, as detectors are typically retrained periodically.


\begin{center}
\fcolorbox{black}{gray!10}{\parbox{.9\linewidth}{\textit{\textbf{Take Away}: TIF slows down the aging of detectors in each feature space and has significant performance gains in the years just after deployment.}}}
\end{center}




% \begin{figure}
%     \centering
%     \setlength{\abovecaptionskip}{0cm}
%     \includegraphics[width=1.0\linewidth]{Figure/RQ2.pdf}
%     \caption{The variance in similarity between malware feature representations generated by different detectors in closed-world and open-world scenarios and those from the training set. \textit{Retrained} refers to detectors retrained at each time point with newly labeled samples.}
%     \label{fig:rq2}
% \end{figure}

\subsection{Robustness in Different Drift Scenarios (RQ2)}
\label{rq2}
Invariant training aims to help malware detectors learn stable representations across drift scenarios over time. To evaluate this, we separate the drift factors, i.e., the evolution of existing malware families and the emergence of new malware families, and construct two test scenarios: a closed-world scenario with only known families and an open-world scenario with novel families. We segment the test environment into 10 intervals by release date. Benign samples from matched periods are added to ensure a natural sample distribution.


We use the top-performing DeepDrebin detector to assess representation stability. For each test interval, we compute the cosine similarity between malware feature representations in each test interval and the training set. Figure~\ref{fig:rq2} shows the variance in similarity across intervals. We retrain the detector in each interval with labeled samples to establish baseline representations for comparison. Results indicate that the invariant training framework consistently yields more stable feature representations in closed and open-world scenarios, showing robustness to drift.

\begin{center}
\fcolorbox{black}{gray!10}{\parbox{.9\linewidth}{\textit{\textbf{Take Away}: TIF generates stable feature representations for both evolved variants of existing families and new malware families.}}}
\end{center}





% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{Figure/RQ1.pdf}
%     \caption{Monthly performance of DeepDrebin (a), Malscan (b) and BERTroid (c) feature spaces for the first test year after deployment (2015), with all models initially trained on 2014 samples. \textit{Retrained} indicates detectors updated monthly by incorporating that month's labeled test samples into the original training set.}
%     \label{fig:rq1}
% \end{figure}


% To answer this question, we decouple the factors that lead to distributional drift in our test set based on the source of the drift, i.e., the evolution of existing malware families and the emergence of new families, and construct two targeted test environments, i.e., closed-world and open-world based drift scenarios. For the former, the test set contains only malicious families already present in the training set, and for the latter, only unseen families. Additionally, given the inherent trade-off between accuracy and robustness to drift~\cite{tradeoff}, we must ensure that improving robustness does not negatively impact the model's performance on non-drifted samples. Therefore, we also evaluated performance on a validation set that follows the same i.i.d. distribution as the training set. Table  presents the F1 score in non-drifted, closed-world and open-world scenarios.

% For existing families, models without TIM consistently exhibited performance degradation across the test set, indicating that malware evolution is a persistent challenge. After incorporating invariant training, the F1 score increases by xx\% and FNR decreases by xx\% for each test year. Furthermore, the emergence of new families significantly reduced the performance of all baseline models. Although the models were trained on the discriminative features of the training set, the appearance of new malware families increased the rate of ineffective discriminative features, leading to performance degradation. TIM mitigated this degradation to some extent by learning invariant features that represent core malicious behaviors in the training set. Finally, on a drift-robust basis, adding TIM does not significantly affect the learning of discriminative features in the training set, with a maximum performance change of less than xx\%.




\subsection{Effective Invariant Feature Learning (RQ3)}
\label{rq3}
We evaluate the framework’s ability to learn invariant features. Section \ref{motivation: failure} shows that ERM models underperform by relying on unstable features. To quantify stable and discriminative feature learning, we define the Feature Contribution Score (FCS) for each feature $f_j$ as follows:
\begin{equation}
    % FCS_j = r(f_j, S^{\prime}) \cdot IS_j,
    FCS_j = \left|r\left(f_j, S_m\right)-r\left(f_j, S_b\right)\right| \cdot IS_j,
\end{equation}
where $r(f_j, S_m)$ and $r(f_j, S_p)$ is the active ratio of feature $f_j$ in malware and benign category respectively and $IS_j$ is its importance score via integrated gradients (IG) with the malicious class as the target. For model $\mathcal{M}$, its discriminative ability is the sum of all FCS values, with higher scores indicating greater focus on discriminative features. We conduct interpretable Drebin feature space experiments to visually assess this capability using closed and open-world settings, as outlined in Section~\ref{rq2}. Results in Table~\ref{tab:rq3} show that invariant training significantly raises FCS, guiding the model to more stable and discriminative features, thus enhancing robustness.

\begin{figure}[hbt!]
    \centering
    \begin{subfigure}[t]{0.48\textwidth}  
        \includegraphics[width=0.9\textwidth]{Figure/similarity_variance_malware_exist_bar.pdf}
        \caption{Variance of representation similarity in closed-world setting}
    \end{subfigure}
    \begin{subfigure}[t]{0.48\textwidth}  
        \includegraphics[width=0.9\textwidth]{Figure/similarity_variance_malware_open_bar.pdf}
        \caption{Variance of representation similarity in open-world setting}
    \end{subfigure}
    \caption{The variance in the similarity between malware feature representations generated by different detectors in closed-world (a) and open-world (b) scenarios and those from the training set. \textit{Retrained} refers to detectors retrained at each time point with newly labeled samples.}
    \label{fig:rq2}
\end{figure}

We also retrain the detector with TIF then analyze the top 10 important features and tracked their discriminability. As shown in Figure~\ref{fig:feature_diff_10_irm},  invariant training improved test performance, with F1 scores exceeding those of the original model and prioritized features demonstrating greater stability. Newly highlighted permissions, such as \verb|GET_TASK| and \verb|ACCESS_FINE_LOCATION| show stronger correlations with malicious behavior, confirming that invariant training helps shift focus to more robust features.

\begin{center}
\fcolorbox{black}{gray!10}{\parbox{.9\linewidth}{\textit{\textbf{Take Away}: TIF enables the detector to learn stable, discriminative features from the training set.}}}
\end{center}

\begin{figure}
    \centering
    % \setlength{\abovecaptionskip}{0cm}
    \includegraphics[width=1.0\linewidth]{Figure/feature_diff_10_irm.pdf}
    \caption{Discriminability for the Top-10 important features after invariant training. F1 Score (Drebin) denotes the performance of the model trained based on Section~\ref{motivation: failure} and F1 Score (Drebin + TIF) denotes the result after trained by invariant training framework TIF.}
    \label{fig:feature_diff_10_irm}
\end{figure}


% We evaluate the proposed framework's ability to learn invariant features. The empirical analysis in Section \ref{motivation: failure} shows that ERM-trained models fail due to their reliance on unstable, weakly discriminative features. Repeating the same setup with the TIM framework, we retrain the model, focusing on the top 10 important features and their discriminative power over the test intervals. The results show that TIM significantly improves F1 scores, mitigating early performance degradation. Moreover, compared with Figure.~\ref{fig:importance}, the selected features demonstrate more stable discriminative power. Newly highlighted permissions, such as \texttt{GET\_TASK} and \texttt{ACCESS\_FINE\_LOCATION} show stronger correlations with malicious behavior, confirming that invariant training helps shift focus to more robust features.

% Additionally, we evaluate the proposed framework's ability to learn invariant feature representations. Based on the type of invariance, we divided the malicious test samples into two groups: those with families present in the training set and those without. The test samples were strictly ordered by release date and split into 10 equal-length intervals. 


\subsection{Ablation Study}
This section evaluates the robustness of each component through an ablation study. Five configurations are tested: the base model, +MPC1, +MPC1 +MPC2, +MPC1 +IGA2, and +MPC1 +IGA2 +MPC2, where MPC1/MPC2 represent multi-proxy contrastive learning, and IGA2 denotes invariant gradient alignment. Table~\ref{tab: ablation} shows the AUT(F1, 12m) results for each setup with the Drebin detector.

In stage one, MPC1 refines intra-environment representations, surpassing the baseline despite minor drops in the final year. Adding MPC2 and IGA2 improves generalization by aligning gradients and learning global features, increasing resilience to drift. The full configuration achieves the highest robustness by unifying feature learning and filtering stable, risk-minimizing features.

\input{Table/RQ3}
\input{Table/Ablation}
\input{Table/Env}

\subsection{Temporal Environment Granularity Selection}
\label{env seg}
In invariant learning, environment segmentation is critical for exposing uncertainty to the model while maintaining sufficient samples per environment for effective learning. Using a one-year training set, we evaluate three segmentation granularities: monthly, quarterly, and equal-sized splits ($n=4$, $8$, and $12$). Table~\ref{tab: env} reports the AUT(F1, 12m) scores for each method across the test phase. Equal-sized splits often increase label imbalance, hindering robust representation learning. Fine-grained partitioning improves feature discrimination but reduces per-batch samples as environments increase, complicating cross-environment alignment. Coarser granularity supports long-term robustness, while finer granularity boosts short-term performance, with partitioning typically guided by validation results, e.g., preferring monthly splits when validated on 2015 samples.


==> History/Introduction.tex <==
\section{Introduction}


In open, dynamic environments, even the most effective malware detectors face significant challenges posed by various forms of distribution drift{}\footnote{For clarity, we use the terms drift, shift, concept drift/shift, and distribution drift/shift interchangeably throughout the text.}, leading to performance degradation~\cite{transcending, cade}. From a conceptual perspective, without reasoning on the underlying representations, there are two main causes of drift in Android malware classification tasks: the evolution of malware behaviors and the emergence of previously unseen malware families that exhibit new behaviors~\cite{pei2024exploiting}. The emergence of new variants and families shifts the fundamental statistical properties of test samples~\cite{tesseract, overkill, transcending, Drift_forensice}, thereby weakening the performance of detectors trained on past patterns~\cite{malware_evolution_update}.

% These variants and new families may change the underlying statistical properties of the input samples at the test time~\cite{tesseract, overkill, transcending, Drift_forensice}, resulting in the underlying representations not being able to generalize to them and weakening the effectiveness of patterns learned by the detector from the training dataset~\cite{malware_evolution_update}.

Recent studies have explored incremental training techniques, which involve detecting new distributions during testing and frequently updating models through active~\cite{tesseract, continuous} or online learning~\cite{droidevolver, online_mal, labelless} to address distribution drift. However, these approaches incur significant labeling and model update costs. Although pseudo-labeling has been used to alleviate labeling burdens, it introduces noise that can lead to self-poisoning models~\cite{labelless, recda}, further complicating the learning process. Therefore, improving the robustness of the model in drifting scenarios is essential to reduce the frequency of model updates. Some studies have attempted to use static feature augmentation or select features that are less sensitive to malware evolution~\cite{scrr, apigraph, overkill}. Yet, these often require specific selection methods tailored to different feature spaces that may underperform as drift sources change. Ideally, a drift-robust detector would emphasize features in the training set that both contribute to high performance and remain stable under drift, thus capturing commonalities across different distributions. However, the current training paradigm inhibits the model's ability to learn such invariance.

% Several works focus on robustness under distributional drift~\cite{scrr}. Some use static feature enhancement to extract new feature spaces from applications that are less sensitive to malware updates~\cite{apigraph, overkill}, typically requiring carefully designed selection methods for specific feature spaces. Others adopt incremental retraining~\cite{tesseract}, periodically detecting new distributions during testing and frequently updating models through strategies like active learning~\cite{tesseract, continuous} and online learning~\cite{droidevolver, online_mal, labelless}. These approaches introduce knowledge from new distributions (e.g., new feature constraints or training data) to help models learn commonalities between old and new knowledge. Thus, a detector’s robustness to drift can be seen as its ability to learn stable, discriminative features that generalize to test samples to represent these commonalities. However, we argue that even without new knowledge, some of such invariant features already exist in the current training set and feature space, but are obscured by the existing training paradigm.

% Several works focus on robustness under distributional drift~\cite{scrr}. Some use static feature enhancement to extract new feature spaces from applications that are less sensitive to malware updates~\cite{apigraph, overkill}. This often requires feature selection tailored to a specific feature space~\cite{svm_ce}. Others adopt incremental retraining~\cite{tesseract}, detecting new distributions emerging during testing, and frequently updating the model through strategies such as active learning~\cite{tesseract, continuous} and online learning~\cite{droidevolver, online_mal, labelless}. While this allows new knowledge (e.g., new training data) to become available over time, the model cannot automatically adapt to drift scenarios when such knowledge is missing. Thus, robustness to drift largely depends on the model’s ability to learn stable and discriminative feature representations during training that can generalize to test samples. We posit that the existing feature space already contains undiscovered such patterns, i.e. invariant features, yet they are often overlooked under current training paradigms.
% To support this conclusion
In this paper, we conduct a comprehensive investigation into learning-based malware detectors. Our findings indicate that even when invariant features representing shared malicious behaviors exist within malware families or variants, detectors struggle to learn these features effectively. This inefficiency can be attributed to the limitations inherent in the empirical risk minimization (ERM) training paradigm. ERM operates under the assumption that training and testing data conform to the same distribution, requiring data shuffling or constructing k-fold cross-validation sets. However, in real-world scenarios, testing data is often collected after the training period~\cite{tesseract}, meaning the shuffled training set fails to capture the sequential transition pattern between training and testing samples, hindering the model's adaptability to the dynamic evolution of malware.

% To support this conclusion, we analyzed real malware source code from different time intervals and found invariances in Android malware evolution. Variants within the same family or across different families with similar malicious goals share some parts of core malicious behaviors, even though implementation details vary due to Android updates or various external factors. These behaviors represent underlying invariant features, providing a foundation for models to learn invariant patterns. We further examined existing learning-based detectors to identify their inefficiency in learning such temporal invariant representations. This stems from the assumption of empirical risk minimization (ERM), which requires training and test data to follow the same distribution. Typically, data is shuffled and evaluated in static settings (e.g., hold-out or k-fold validation). However, in real-world scenarios, test data appears after the training period \cite{tesseract}, meaning that current training methods overlook the learnable dynamics of malware evolution. 


% To support this hypothesis, we first reveal the invariance in Android malware evolution from the source code perspective. For malware of the same family, although they may differ in implementation details due to evolution caused by external factors, their consistent malicious intent ensures that they share a set of core features that represent malicious behavior. In addition, the objectives of malicious behavior are inherently limited~\cite{malradar}. Thus, even if certain families are absent in the training data, their execution may still resemble those in the test data with similar behaviors. These two forms of invariance provide a foundation for the model to learn an invariant paradigm. However, the failure of malware detectors based on empirical risk minimization (ERM) seems to indicate its shortcomings in learning these invariants. This motivates us to revisit its training process and find that the flaws stem from the underlying assumption of ERM, which requires training and test data to follow the same independent and identically distributed (i.i.d.) distribution. One common practice to satisfy this requirement is to shuffle training and testing datasets, and model performance is evaluated in a static setting (e.g., using hold-out or k-fold cross-validation). However, real-world environments necessitate observing test data over time following the training period\cite{tesseract}. Shuffling the training set often leads to the loss of critical information about the dynamics of malware evolution{}\footnote{While we focus on malware, the same reasoning can be applied to goodware too.}, causing the training phase to capture only transient features that are effective for the specific time window of the training data but struggle to generalize to new patterns introduced by evolving malware variants~\cite{EIC}. Angioni et al.~\cite{svm_ce} also found the importance of finding temporal invariant features and proposed a feature stability metric, t-stability, to evaluate the contribution of fluctuations in individual features to the degradation of detector performance. However, this method is based on the direct relationship between feature weights and classification performance of a linear classifier and fails to generalize to a more complex group of features and nonlinear relationships.

Invariant learning theory~\cite{IR_intro} aims to address the shortcomings of ERM by learning invariant features shared across different distributions, which aligns with our objective. This theory promotes the discovery of stable representations by dividing training data into distinct subsets or ``environments'' and encouraging the model to minimize differences between them. However, common invariant learning methods typically require prior knowledge of environment labels that reveal unstable features~\cite{environment_label, env_label} and assume the encoder is capable of learning rich, high-quality representations~\cite{yang2024invariant}. These requirements and assumptions are not trivial for malware detection, where drift arises from various non-obvious factors, compounded by imbalanced sample distributions and a diverse feature space that complicates representation learning.

% The above observations motivated us to extend the empirical risk minimization (ERM) training strategy to learn temporally invariant features for malware detectors. This aligns with invariant learning theory, which promotes the discovery of stable representations by dividing training data into distinct subsets, or "environments," and encouraging the model to minimize inter-environmental differences. However, this approach requires prior knowledge of environment labels to expose known unstable features~\cite{environment_label, env_label} and an encoder capable of learning rich representations to identify stable components~\cite{yang2024invariant}. In malware detection, these conditions are more challenging due to distribution drift influenced by multiple factors, unbalanced sample distributions, and non-intuitive features.

This paper presents a temporal invariant training framework, TIF, designed for malware detectors to facilitate the learning of invariant features under distribution drift. Specifically, we partition the training data according to the natural release times of applications, thereby exposing the complex instability of malware evolution over time and avoiding the reliance on prior environment labels. In the context of binary classification tasks, we identify that learning homogeneous representations for a merged multi-family malware class is suboptimal. Recent works have focused on constructing positive relationships within individual malware families to enhance feature representations~\cite{continuous}. However, such an overly fine-grained approach often exacerbates sample imbalance issues. To address this, we propose a multi-proxy contrastive learning module. In our proposed framework, each proxy is a representation of a similar subset within the class, with dynamic updates to multiple proxies that aim to capture feature representations reflective of the application's true semantics. Additionally, we design an invariant gradient alignment module grounded in invariant learning theory, ensuring that the encoder generates similar gradients for samples belonging to the same class across different environments, thereby promoting the learning of high-quality, cross-environment invariant representations. Our solution is orthogonal to existing robust malware detectors; it does not depend on new feature spaces, requires no changes to existing model architectures, and can be applied to any learning-based detector. The main contributions of this paper are as follows:

% This paper aims to propose a unified invariant training framework for Android malware detectors to learn invariant representations in drift scenarios. We first partition the training data by application release dates, preserving distributional changes without focusing on a single drift factor. Additionally, learning homogeneous representations for mixed malware families is suboptimal. Recent work~\cite{continuous} on fine-grained positive relations for each family may lead to excessive relations and worsen class imbalance. We propose a multi-proxy contrastive learning module that learns multiple dynamic proxy representations for each category, aligning samples with similar proxies to avoid forcing dissimilar distributions together. Building on the challenges of invariant learning, an invariant gradient alignment module is designed based on this theory. It ensures that the encoder generates similar gradients for same-class samples from different environments when processed by the same classifier. To this point, we finally develop an invariant training framework, TIF, for malware detection. Through a two-stage training process, it amplifies and compresses unstable information across environments, enabling the encoder to learn time-invariant malware representations. The proposed solution is orthogonal to existing drift-robust malware detectors. It does not rely on new feature spaces, requires no modifications to existing model architectures, and can be applied to any learning-based detector. The main contributions of this paper are as follows:

% Based on the above observations, we propose that ERM training can be extended to learn temporally invariant features for malware detection. Invariant learning~\cite{IRM_training} offers a potential solution by partitioning the training set into different environments to expose instabilities, thereby encouraging the model to discover cross-environment invariant representations by minimizing differences between environments. Inspired by this theory, an intuitive approach is to restructure the training set to incorporate the temporal evolution of malware. Specifically, we sample training data from different time-based subsets (environments) of application release dates, with each subset satisfying ERM's prerequisites. The temporal isolation between subsets naturally preserves the distribution shifts in malware. The training objective is establishing invariant feature representations between each subset while minimizing their empirical risk. This scheme also addresses the limitation of applying invariant learning theory, i.e., the acquisition of environment labels often relies on a priori knowledge and requires knowing which features the model is wrongly focusing on. Here, application timestamps naturally provide environment delineation labels while retaining information about distribution changes across time. 

% The above intuition leads us to propose TIM, an invariant training framework for Android malware detection. The framework leverages application release dates to naturally construct training environments. We then designed two core components for invariant training: Multi-Proxy Contrastive Learning and Invariant Gradient Alignment. The former models rich feature representations within both normal and malicious categories, aiming to maximize the learning of discriminative information from the training set. The latter aligns the classification gradients of same-class samples across environments based on Invariant Risk Minimization (IRM). Through these two components, the invariant training framework extracts invariant feature abstractions from the diverse representations of each environment. The proposed solution is orthogonal to existing drift robust malware detectors. It does not rely on a new feature space and needs no modifications to the existing model structure, can be applied to any learning-based detector. The main contributions of this paper are as follows:

\begin{itemize}
    \item We define invariance in malware evolution, positing that learning stable and discriminative invariant representations is key to mitigating malware vulnerability in drift scenarios.
    \item We propose a first temporal invariant learning framework, TIF, for malware detectors, which can be integrated with arbitrary detectors to learn invariant representations over time by exposing and compressing unstable information in drifts.
    % \item We propose a temporal invariant learning framework for malware detection tasks that aids arbitrary detectors in learning representation invariance in software evolution by exposing and compressing unstable information in malware drift.
    \item We carefully design multi-proxy contrastive learning and invariant gradient alignment modules to model complex distributions within malware and encourage the model to learn high-quality and stable representations across temporal variations.
    \item We construct a 10-year dataset\footnote{We will open source the dataset metadata and code repository to foster reproducibility studies.} and a series of experiments to evaluate the robustness of the TIF across various drift scenarios and feature spaces. The results show that TIF effectively slows the detector's degradation and generates invariant representations that outperform state-of-the-art methods.
\end{itemize}


% Others, instead, dynamically update models following incremental retraining~\cite{tesseract}, active learning~\cite{tesseract, continuous}, and online learning~\cite{droidevolver, online_mal, labelless} strategies. By periodically detecting new distributions that appear at test time~\cite{transcending}, the model is retrained to always have a valid feature representation relative to the test set. Essentially, these approaches learn new features, new distribution of existing features, or a combination thereof, as new knowledge (e.g., new training data) becomes available over time~\cite{overkill}. When this new knowledge (i.e., new training data) is missing, the models fail to adapt to drift scenarios as they fail to learn discriminative \emph{and} stable features that remain invariant over time. We argue existing feature space already contains as yet undiscovered learnable invariant information that is masked under existing training paradigms.

% Based on this intuition, we propose an invariant training strategy for Android malware detection. The solution naturally constructs the training environment for exposing temporal-varying features based on the release time of applications. After that, we elaborate on two core modules for invariant training, i.e., invariant representation alignment and invariant gradient alignment, which enable the model to extract uniform and invariant feature abstractions from the rich feature representation information learned through the dual alignment of the encoder and classifier. The proposed solution is orthogonal to existing drift robust malware detectors. It does not rely on a new feature space and needs no modifications to the existing model structure. We evaluate its robustness against new malware families and variants of existing families on datasets with different drift levels and time span, which significantly improves the performance of the malware detector in drifting scenarios. The main contributions of this paper are as follows:

    % \item We evaluated the invariant-enhanced model performance on datasets with various drift levels and periods, with F1 scores improving by up to 8.10\% (4.63\% on avg), FNR reducing by up to 49.89\% (17.55\% on avg) and AUT (on F1 score) up to 4.75\% (overall about 3\%) over 5 years.




==> History/Methodology.tex <==
\section{Methodology}

\subsection{Preliminary}
\subsubsection{Notations}
We use uppercase and lowercase letters to denote matrices and vectors, respectively; $|\mathcal{D}|$ represents the total number of elements in set $\mathcal{D}$. 

\begin{figure*}
    \centering
    % \setlength{\abovecaptionskip}{0cm}
    \includegraphics[width=1.0\linewidth]{Figure/model_architecture.pdf}
    \caption{The proposed invariant training framework and its core components}
    \label{fig:model_architecture}
\end{figure*}

\subsubsection{Problem setting}
In the problem of Android malware detection, we divide the samples $x \in \mathbb{R}^{d}$ into two parts: the first part is the labeled current moment training data $\mathcal{D}_{tr} = {(x_i^{tr},y_i^{tr})}^{|\mathcal{D}_{tr }|}_{i=1}$, where $y_{i}^{tr} \in \{0, 1\}$ represents the labels for benign and malicious applications. All training data are from a specific period $\mathcal{T}_{tr}$, and each sample $x_i^{ts}$ contains its corresponding release timestamp $t_i^{tr}$. The second part is the upcoming unlabeled test data $\mathcal{D}_{ts}$, the timestamps of whose samples $t_i^{ts}$ are strictly from future moments compared to $\mathcal{T}_{tr}$ and they appear progressively over time. We assume that the training and test data share the same label space and have unknown semantic similarity, but show a certain degree of difference in data distribution. These distribution differences lead to degradation of the performance of the currently deployed malware detectors on the test data. The model is represented as $\mathcal{M} = c \circ \phi$, where $c$ denotes the classifier and $\phi$ is the feature encoder. This paper aims to help the encoder in arbitrary detectors capture invariant semantic information shared with unseen test data based on training data. 




\subsection{Overall Architecture}
Section~\ref{motivation: failure} illustrates the importance of learning temporally stable and discriminative features to improve robustness against distribution drift. Based on this, we propose a temporal invariant training method, which can be integrated into arbitrary malware detectors. This method enables the encoder to capture rich discriminative information from the training data, and then suppress the unstable cross-environment factors through invariant risk minimization, enhancing robustness in drift scenarios. The training process relies on two core components: \textbf{Multi-Proxy Contrastive Learning (MPC)}: This component models the diversity in the representations of benign samples and malware using dynamically updated proxies. It specifically encodes the complex semantic information of multi-family malware into the embedding space, learning more compact and faithful embeddings that fully expose the latent discriminative information in the training data. \textbf{Invariant Gradient Alignment (IGA)}: This component uses invariant risk minimization (IRM) to reduce gradient variance across different environments for samples of the same class, encouraging the encoder to learn a unified representation for all environments (i.e., time intervals).

Figure~\ref{fig:model_architecture} illustrates the overall framework of the proposed method. We first divide Android applications into multiple non-overlapping environments based on their release time. Since the prerequisite for learning invariant features is the model’s ability to construct rich representations of potentially useful features, the invariant training process is divided into two stages: 
\begin{itemize}
    \item Discriminative Information Amplification Stage: In this stage, MPC is independently applied within each environment while minimizing empirical risk, allowing the shared encoder to integrate discriminative information from each environment.
    \item Unstable Information Compression Stage: Building on the model trained in the previous stage, MPC is applied across all environments to align feature representations. Following this, the IGA fine-tunes the encoder using IRM through the dummy classifiers to suppress unstable information.
\end{itemize}

% Section 3.2 illustrates the importance of learning stable and discriminative features for drift robustness enhancement, centred on the ability of the encoder to adequately capture the rich discriminative information in the training set, and later compress cross-environmental instabilities through invariant learning. Based on this, we propose a temporal invariant training method that can be integrated into an arbitrary malware detector to help it learn stable and discriminative information to enhance its robustness in drifting scenarios. The training process split into two key phases: \textbf{Discriminative information amplification}: We introduce multi-proxy contrastive learning to encode the complex semantic information of multi-family malware into the embedding space. Using multiple dynamically updated proxies, we model the natural diversity within benign and malicious samples, thereby learning more compact and faithful embeddings that fully expose the potential discriminative information in the training data. \textbf{Unstable information suppression}: This module suppresses unstable transient features through invariant risk minimization (IRM), reducing the variance of similar samples across different environments and encouraging the encoder to learn temporal-invariant feature representations.

% Motivated by the above considerations, we propose a temporal invariant training method that can learn stable and discriminative information from the training set in an end-to-end manner. This approach can be integrated into any malware detector to enhance its robustness in drift scenarios.  

% As shown in Figure.\ref{fig:model_architecture}, the overall architecture first divides the training samples into multiple disjoint environments. Discriminative information within each environment is amplified through multi-proxy contrastive learning to motivate the encoder to learn the rich discriminative information in each environment. Afterwards, unstable transient features are suppressed through invariant risk minimization, ensuring that the final embeddings primarily capture stable and discriminative features.

\subsection{Training Environments Segmentation}
\label{environment_split}
Segmenting the training environment requires exposing unstable information. Malware distribution drift arises from multiple factors, such as application market demands or Android version updates. Dividing the training environment based on application release times effectively captures this mix of unknown causes. For a dataset with timestamps from $T_{\min}$ to $T_{\max}$, and a chosen time granularity $\Delta$, samples are divided into $t$ time windows, each representing an environment $e \in \mathcal{E}$, where $|\mathcal{E}| = t$. The resulting training set is an ordered multiset, $\mathcal{D} = \{D_1,D_2,...,D_t\}$, with each environment $D_t$ containing $|D_t|$ samples. A sample $x_i$ with timestamp $t_i$ is assigned to an environment using:
\begin{equation}
\mathcal{E}(x_i)=\left\lfloor\frac{t_i-T_{\min }}{\Delta}\right\rfloor.
\end{equation}
As the environment index increases, the corresponding timestamps move closer to the present. The choice of time granularity depends heavily on dataset sparsity and involves a trade-off: finer granularity reveals detailed distribution patterns but risks insufficient sample size for effective representation learning, while coarser granularity may overlook distribution shifts. A balanced granularity can mitigate these issues but requires careful consideration of label distribution within each environment to prevent misalignment in learned representations. Section~\ref{env seg} examines the impact of different granularity choices.

\subsection{Multi-Proxy Contrastive Learning}
\label{multi-proxy contrastive learning}
Malware families have distinct distributions and imbalanced sample sizes, complicating malware category modeling in the embedding space. Benign samples may also display complex feature distributions due to factors like geographic location or user behavior. Treating all relationships within a category equally can exacerbate imbalances, while overly homogenizing samples overlooks valuable information. Thus, effective discrimination requires balancing the complex pairwise relationships within each category to ensure high-quality representations that capture sample diversity.

To address this, we design a multi-proxy contrastive learning method, where each proxy represents a subset of samples with similar behaviors or structures. This approach enables the encoder to capture finer-grained features within each class, rather than treating all benign or malicious samples as homogeneous groups.



% Modeling the malware category with different kinds of malware families which have diverse distributions and imbalanced sample sizes is challenging. Therefore, it is crucial to capture this kind of diversity within each class to better align the complex positive pair relationships among samples from the same category. To this end, we propose a multi-proxy contrastive learning method, where multiple proxies are dynamically obtained within each class. Each proxy represents a subset of samples with similar behavior or structural characteristics. This allows the encoder to capture more fine-grained features for each category at this stage, rather than naively treating all benign/malicious samples as a homogeneous group.

For a given batch of samples $\mathbf{X}_c \in \mathbb{R}^{|\mathcal{B}_c| \times d}$ from category $c$ , where $|\mathcal{B}_c|$ is the batch size and $d$ is the feature dimension, we randomly initialize $K$ proxies for both goodware and malware categories. Each sample is then assigned to relevant proxies. In this multi-proxy setup, avoiding dominance by any single proxy helps mitigate noise. Inspired by the Sinkhorn~\cite{sinkhorn} algorithm, we compute a probability matrix $\mathbf{W}_c$ for proxies within category $c$, assigning a weight $w_{ij}$ to proxy $j$ for each sample $x_i$ as follows:
\begin{equation}
w_{i j}^{(c)}=\frac{u_i \cdot \exp \left(\frac{sim(\mathbf{x}_i, \mathbf{P}_c^{(j)})}{\epsilon}\right) \cdot v_j}{\sum_{i=1}^{|\mathcal{B}_c|} \sum_{j=1}^K u_i \cdot \exp \left(\frac{sim(\mathbf{x}_i, \mathbf{P}_c^{(j)})}{\epsilon}\right) \cdot v_j},
\end{equation}
where $\epsilon$ is a temperature parameter controlling the smoothness of the assignment. $sim(\mathbf{x}_i, \mathbf{P}_c^{(j)})$ represents the dot-product similarity between the sample and the proxy. $u_i$ and $v_j$ are auxiliary normalization factors to ensure that all assigned weights satisfy a doubly-normalized constraint, adjusted iteratively through row and column scaling.

To reduce the complexity, the top-N proxies with larger weights are selected here to participate in the computation of the proxy loss. Thus, for the sample over the selected proxies, the proxy alignment loss is denoted as:
\begin{equation}
\mathcal{L}_{pal}=-\frac{1}{|\mathcal{B}_c|} \sum_{c=1}^C \sum_{i=1}^{|\mathcal{B}_c|}\left(\sum_{j=1}^N \mathbf{W}_c^{(i, j)} \cdot \log \left(p_{i j}^c\right)\right),
\end{equation}
where $p_{i j}^c$ is the softmax probability calculation for sample $i$ and proxy $j$ within each class $c$, represent as follow:
\begin{equation}
p_{i j}^c=\frac{\exp \left(sim(\mathbf{x}_i, \mathbf{P}_c^{(j)}) / \tau\right)}{\sum_{k=1}^N \exp \left(sim(\mathbf{x}_i, \mathbf{P}_c^{(k)}) / \tau\right)},
\end{equation}
where a temperature parameter $\tau$ is applied to scale the similarities.

The distribution of proxies determines the diversity of distributions the embedding can represent. To enhance the diversity, we introduce a proxy contrastive loss that disperses proxies within the same class. Each proxy serves as a positive sample for itself, while other proxies in the class are negatives. To distinguish proxy-to-proxy similarities from sample-proxy similarities, we define the former similarity as $sim_p(\mathbf{P}_c^{(i)}, \mathbf{P}_c^{(i)})$ and the proxy contrastive loss is given as:
\begin{equation}
\mathcal{L}_{pcl}=-\frac{1}{K} \sum_{c=1}^C \sum_{i=1}^K\left(\log \left(\tilde{p}_{ij}^c\right)\right)
\end{equation}
Similarly, $\tilde{p}_{ij}^c$ denotes the computation of softmax probability between proxy $i$ and proxy $j$ in category $c$, i.e:
\begin{equation}
\tilde{p}_{ij}^c = \frac{\exp \left(sim_p(\mathbf{P}_c^{(i)}, \mathbf{P}_c^{(i)}) / \tau\right)}{\sum_{j=1}^K \exp \left(sim_p(\mathbf{P}_c^{(i)}, \mathbf{P}_c^{(k)}) / \tau\right)}.
\end{equation}

During training, proxies in each category are progressively updated to adapt to the evolving distribution of applications. Updates are performed using a momentum strategy, where momentum is derived from the weighted sum of the previously obtained weight matrix and the samples associated with each proxy. The updated proxies $\mathbf{P}_c^{\prime}$ of class $c$ are computed as follows:
\begin{equation}
\mathbf{P}_c^{\prime}=\gamma \mathbf{P}_c+(1-\gamma) \mathbf{W}_c^T \mathbf{X}_c,
\end{equation}
where $\gamma$ is the momentum coefficient controlling the update rate. Therefore, we can obtain the multi-proxy contrastive loss as the training objective in this module, which can be formalized as:
\begin{equation}
\mathcal{L}_{MPC} = \mathcal{L}_{pal} + \lambda \cdot \mathcal{L}_{pcl}
\end{equation}
where $\lambda$ balance the weight of these two loss functions.




\subsection{Invariant Gradient Alignment}
Section~\ref{learn_invariant_feature} discusses the prerequisites for learning invariant features, specifically, the need for environment segmentation to expose unstable information and for rich feature representations. Therefore, based on the definition of Invariant Risk Minimization (IRM) in Section~\ref{invariant_learning}, our goal is to encourage encoders that can learn rich feature representations to further focus on the stable part of them. So here it is necessary to ensure that the representations generated by the encoder for the same class of samples in different environments produce similar gradients in the classifier. To achieve this, we construct an invariant gradient alignment module based on IRMv1, as proposed by Arjovsky \textit{et al.}~\cite{IRM_training}, which is used to strengthen the model's focus on invariant features. The objective function is described as Eq.\ref{grad_align}:
\begin{equation}
\label{grad_align}
\mathcal{L}_{IGA} = \frac{1}{|\mathcal{E}|} \sum_{e \in \mathcal{E}} \left\|\nabla_{s_{e} \mid s_{e}=1.0} R^{e}(s_e \circ \phi)\right\|^2
\end{equation}
Here, $s_{e}$ acts as a scalar, serving the role of a dummy classifier, set to 1.0 and updates through gradient backpropagation. $\mathcal{L}_{grad}$ evaluates how adjusting $s_e$ minimizes the empirical risk in environment $e$. $R^e(s_e \circ \phi)$ is represented as Eq.~\ref{risk_minimization}:
\begin{equation}
\label{risk_minimization}
R^{e}(s_{e} \circ \phi)=\mathbb{E}^{e}\left[\mathcal{L}_{CLS} \left(s_{e}\left(\phi\right(x\left)\right), y\right)\right],
\end{equation}
where $\mathcal{L}_{CLS}$ denotes the classification loss function used in the current environment, such as binary cross-entropy for malware detection. This loss is computed following standard ERM training. The term $\phi(x)$ represents the output of the shared encoder for samples $x, y \sim p(x, y|e)$ from environment $e$. The gradient penalty term encourages uniform feature representation by aligning gradients of classifiers across environments, thereby promoting consistent model performance.

\subsection{Invariant Training Framework}
\label{invariant training}
Gradient adjustment for invariant learning classifiers relies heavily on the encoder’s ability to learn rich representations~\cite{rich}. Starting classifier training from random initialization can cause IRM to converge to local optima. To address this, we propose a two-stage training strategy to capture a broad set of useful features before applying invariant learning.

\subsubsection{Discriminative Information Amplification}
In the first stage, we perform ERM training independently for each environment as the encoder's initialization. The multi-proxy contrastive learning module is applied to each environment respectively to fully exploit the discriminative features within. The optimization objective in this stage is defined as Eq.\ref{erm loss}:
\begin{equation}
\label{erm loss}
\mathcal{L}_{ERM} = \frac{1}{|\mathcal{E}|} \sum_{e \in \mathcal{E}} (\mathcal{L}_{CLS}^e + \alpha \cdot \mathcal{L}_{MPC}^e),
\end{equation}
where $\mathcal{L}_{CLS}^e$ and $\mathcal{L}_{MPC}^e$ denote the classification loss and multi-proxy contrastive loss for environment $e$, respectively. Jointly minimizing the empirical risk across all environments in this stage enables the encoder to learn diverse feature representations, creating a robust foundation for subsequent invariant training.

\subsubsection{Unstable Information Suppression}
To mitigate overfitting to environment-specific features from the earlier stage, we reset the optimizer’s parameters before the second training phase. This reset allows the model to refocus on the objectives of invariant learning. In this phase, we first apply a multi-proxy contrastive loss across all samples to enhance class representation learning. Next, invariant gradient alignment is used to harmonize classification gradients across environments. The updated optimization objective is defined in Eq.~\ref{irm loss}:
\begin{equation}
\label{irm loss}
\mathcal{L}_{IRM} = \mathcal{L}_{CLS} + \alpha \cdot \mathcal{L}_{MPC} + \beta \cdot \mathcal{L}_{IGA},
\end{equation}
In training, the hyperparameters $\alpha$ and $\beta$ balance the contributions of each loss term. This two-stage approach enables the model to first capture a broad feature set, then refine it for cross-environment invariance, enhancing generalization under distribution shifts. The pseudo-code of the training process is shown in Appendix~\ref{alg1}.

% \input{Algorithm/Invariant_training}









==> History/Motivation.tex <==
\section{Motivation}
\begin{figure*}
    \centering
    \setlength{\abovecaptionskip}{0cm}
    \includegraphics[width=1.0\linewidth]{Figure/motivation_sample.pdf}
    \caption{(a), (b), and (c) show real code snippets from an early Airpush version, a later Airpush version, and the Hiddad adware family. Airpush's core behavior includes: (1) get ad data from a specific URL, (2) asynchronous execution to avoid user interruptio, and (3) push ads continuously through the background service. (a) and (b) demonstrate that both Airpush versions share invariant behaviors, with similar API calls and permissions despite implementation differences. Hiddad, while skipping step (2) for simpler ad display, shares steps (1) and (3) with Airpush, especially the newer version.}
    \label{fig:motivation_sample}
\end{figure*}

\subsection{Invariance in Malware Evolution}
% Malware families commonly evolve to circumvent new detection techniques and security measures, resulting in constant changes in their code implementations or API calls. These changes cause the feature space, extracted from applications, to gradually deviate from the initial decision boundaries of malware detectors, thereby significantly degrading detection performance. However, we have identified that during the evolution of malware, core malicious behaviors and execution logic exhibit a certain degree of invariance. This invariance is reflected in the training set through specific intents, permissions, and function calls, which are captured by feature extraction techniques. We categorize this invariance into two types: intra-family invariance and inter-family invariance. 
Malware families commonly evolve to circumvent new detection techniques and security measures, resulting in constant changes in their code implementations or API calls to bypass detection. This leads to drifts in the feature space and a decline in detection accuracy. Yet, we argue that during the evolution of malware, core malicious behaviors and execution patterns remain partially invariant, captured in training data through intents, permissions, and function calls. We define these invariances as intra- and inter-family invariance.
\begin{itemize}
    \item Intra-family invariance: While versions within a malware family may vary in implementation, their core malicious intent remains relatively stable.
    \item Inter-family invariance: Certain malicious behavior patterns are consistent across different malware families. As malware trends shift, even new families emerging after detector training may share malicious intents with families in the training set.
\end{itemize}
To illustrate invariant malicious behaviors in drift scenarios, we select APKs from Androzoo\footnote{https://androzoo.uni.lu} and decompile them using JADX\footnote{https://github.com/skylot/jadx} to obtain .java files. Our analysis focuses on core malicious behaviors in the source code. For intra-family invariance, we use versions of the Airpush family, known for intrusive ad delivery, from different periods. For inter-family invariance, we examine the Hiddad family, which shares aggressive ad delivery and tracking tactics but uses broader permissions, increasing privacy risks. Figure.\ref{fig:motivation_sample} shows code snippets with colored boxes highlighting invariant behaviors across samples. While Airpush uses asynchronous task requests, Hiddad relies on background services and scheduled tasks to evade detection.

% To highlight the invariance of malicious behaviors in drift scenarios, we selected real APK files from Androzoo~\footnote{https://androzoo.uni.lu} platform and decompiled them using the jadx tool~\footnote{https://github.com/skylot/jadx} to obtain their corresponding .java files. The invariance analysis is conducted on the core malicious behaviors represented in the source code. For intra-family invariance, we used the long-standing Airpush malware family as an example, selecting versions from different periods, which is known for its intrusive ad delivery. For inter-family invariance, we chose the Hiddad adware family, which emerged later. Airpush and Hiddad rely on aggressive ad delivery and user tracking, but Hiddad uses broader permissions, violating more privacy. Figure.\ref{fig:motivation_sample} presents code snippets from these malware families, with colored boxes highlighting the invariant malicious behaviors shared across different family samples. Since Hiddad prioritizes ad delivery via background services and scheduled tasks to avoid suspicion and detection, it omits the asynchronous task requests used in step two by Airpush.

Figure~\ref{fig:motivation_sample}(a)\footnote{MD5: 17950748f9d37bed2f660daa7a6e7439} and (b)\footnote{MD5: ccc833ad11c7c648d1ba4538fe5c0445} show core code from this family in 2014 and later years, respectively. The 2014 version uses \verb|NotifyService| and \verb|TimerTask| to notify users every 24 hours, maintaining ad exposure. The later version, adapting to Android 8.0’s restrictions, triggers \verb|NotifyService| via \verb|BroadcastReceiver| with \verb|WAKE_LOCK| to sustain background activity. In Drebin’s~\cite{Arpdrebin} feature space, these invariant behaviors are captured through features like \verb|android_app_NotificationManager;notify|, \verb|permission_READ_PHONE_STATE| and so on. Both implementations also use \verb|HttpURLConnection| for remote communication, asynchronously downloading ads and tracking user activity, and sharing Drebin features such as \verb|java/net/HttpURLConnection| and \verb|android_permission_INTERNET|.

Similarly, Figure.~\ref{fig:motivation_sample}(c)\footnote{MD5: 84573e568185e25c1916f8fc575a5222} shows a real sample from the Hiddad family, which uses HTTP connections for ad delivery, along with \verb|AnalyticsServer| and \verb|WAKE_LOCK| for continuous background services. Permissions like \verb|android_permission_WAKE_LOCK| and API calls such as \verb|getSystemService| reflect shared, cross-family invariant behaviors, whose learning would enhance model detection across variants.

Capturing the core malicious behaviors of Airpush aids in detecting both new Airpush variants and the Hiddad family, as they share similar malicious intents. These stable behaviors form consistent indicators in the feature space. However, detectors with high validation performance often fail to adapt to such variants, underscoring the need to investigate root causes and develop a drift-robust malware detector.

% Based on this analysis, learning features that represent the core malicious behaviors of the Airpush family not only aids in detecting new Airpush variants but also helps in identifying the Hiddad family. However, malware detectors trained on historical data often fail to effectively detect these malicious samples. Even if the model achieves near-perfect performance on the validation set, its performance deteriorates significantly over time, prompting us to further investigate the root causes and build a drift-robust malware detector.

\begin{center}
\fcolorbox{black}{gray!10}{\parbox{.9\linewidth}{\textit{\textbf{Take Away}: The feature space of training samples contains invariance within and among malware families to be learned.}}}
\end{center}

% The analysis suggests that learning invariant features from the Airpush family not only aids in detecting newer versions of Airpush but also improves the detection of Hiddad. However, in practice, detectors trained on these features fail to effectively identify such samples, with performance degrading over time despite near-perfect validation set results. This motivates further our exploration of an ideal malware detector that can learn these invariant behaviours and remain robust in its discrimination throughout malware evolution.

% We present several representative pseudo-code implementations of malicious software to demonstrate invariance visually. For intra-family invariance, we selected Rootkit, a common malware family present in both the training and testing phases. This family exploits system vulnerabilities to obtain root privileges, enabling high-privilege operations such as modifying system files or the kernel, and intercepting system calls to mask its behavior, showcasing a deep confrontation with the operating system’s security mechanisms. Rootkit execution can be simplified into three main steps: file hiding, root privilege acquisition, and system call hooking. With the introduction of stricter permission management and security measures in Android 6.0, this family had to rely on more complex kernel-level attacks to maintain stealth. Figure X illustrates two simplified executions of Rootkit before and after this update, with (a) representing the earlier version. While (b) introduces more complex system calls like openat and fork for file and process hiding, it retains the core semantics from (a). Both versions use the \textit{interceptSystemCall()} function to intercept system calls. The earlier version intercepted \textit{readdir} to hide malicious files, whereas later versions achieved more sophisticated file hiding by intercepting \textit{openat}. Additionally, both versions implement system-level privilege escalation. The only difference in the new version is that it intercepts the fork system call, returning an error code to hide the malicious process \textit{com.malicious.app}. 

% Privilege escalation and process hiding are also commonly used by other malware families. Figure (c) shows a pseudo-code from the Spyware family, which specializes in stealing sensitive user information while maintaining stealth. Thus, in terms of execution logic, Spyware shares root privilege escalation and process hiding with Rootkit, but additionally calls \textit{TelephonyManager} to collect SIM card serial numbers and send them to a remote server. This is understandable, as despite the diversity of malware families, core malicious behaviors can be categorized into a limited number of types\cite{malradar}. Therefore, we conclude that stable patterns indicative of malicious behavior exist in the training samples. While new functionalities will inevitably emerge, once these patterns are learned, the malware detector will exhibit some robustness against drift.








% \subsection{The Contribution of Features to Detectors}
% \subsection{Create Ideal Drift-robust Malware Detector}
\subsection{Failure of Learning Invariance}
% \subsubsection{Vanilla Malware Detector}
Let $f_r \in \mathcal{R}$ be a sample in the data space with label $y \in \mathcal{Y} = {0, 1}$, where 0 represents benign software and 1 represents malware. The input feature vector $x \in \mathcal{X}$ includes features $\mathcal{F}$ extracted from $f_r$ according to predefined rules. The goal of learning-based malware detection is to train a model $\mathcal{M}$ based on $\mathcal{F}$, mapping these features into a latent space $\mathcal{H}$ and passing them to a classifier for prediction. The process is formally described as follows:

\begin{equation}
\arg \min _{\theta} R_{erm}\left(\mathcal{F}\right)
\end{equation}
where $\theta$ is the model parameter to be optimized and $R_{erm}(\mathcal{F})$ represents the expected loss based on features space $\mathcal{F}$, defined as:
\begin{equation}
R_{erm}\left(\mathcal{F}\right)=\mathbb{E}[\ell(\hat{y}, y)].
\end{equation}
$\ell$ is a loss function. By minimizing the loss function, $\mathcal{M}$ achieves the lowest overall malware detection error. 

% Let $r \in \mathcal{R}$ represent a sample in the original data space, where the corresponding label is denoted as $y \in \mathcal{Y} = \{0, 1\}$, with 0 indicating benign software and 1 indicating malware. The input feature vector $x \in \mathcal{X}$ comprises features $\mathcal{F}$ extracted from $r$ according to specific rules. The objective of learning-based malware detection schemes is to learn a model $\mathcal{M}$ based on the feature set $\mathcal{F}$, which maps the features into a latent space $\mathcal{H}$ and feeds them into a classifier to generate predictions. The process is formally described as follows:

% However, as malware evolves, the model's performance gradually degrades. This motivates us to explore an ideal malware detector that can consistently maintain strong discriminative power throughout malware evolution.

% To explore the robustness of various features in response to malware evolution and their contribution to the performance of the detector, we define two key properties of the features used for training: stability and discriminability. Therefore, the aforementioned objective encourages the model to learn discriminative features that can minimize the loss function. However, as we know, this objective may fail during the evolution of malware. 

% This optimization objective encourages the model to learn discriminative features that minimize the loss function. However, the aforementioned objective function may fail during the evolution of malware. Therefore, to explore the robustness of various features in response to malware evolution and their contribution to the performance of the detector, we define two key properties of the features used for training: stability and discriminability. Intuitively, an ideal drift-robust malware detector would be designed to learn features that are both stable and discriminative. 


\subsubsection{Stability and Discriminability of Features}
\label{active ratio}
To investigate the drift robustness in malware evolution from the feature perspective, we introduce two key properties of features: stability and discriminability. Stability refers to a feature's ability to maintain consistent relevance across different distributions, while discriminability reflects a feature's capacity to distinguish different categories effectively. Typically, feature analysis relies on model performance and architecture, which may introduce bias in defining these feature properties. Therefore, we propose a modelless formal definition, making it applicable across various model architectures. 

Let $f_j$ represent the $j$-th feature in the feature set $\mathcal{F}$, and $S$ denote the set of all samples. To capture the behavior of feature $f_j$ under different conditions, we compute its active ratio over a subset $S^{\prime} \subseteq S$, representing how frequently or to what extent the feature is ``active'' within that subset. Specifically, for a binary feature space, feature $f_j$ takes values 0 or 1 (indicating the absence or presence of the feature, respectively), the active ratio of $f_j$ in the subset $S^{\prime}$ is defined as the proportion of samples where $f_j$ is present, which is defined as Eq.~\ref{active ratio}:
\begin{equation}
\label{active ratio}
r\left(f_j, S^{\prime}\right)=\frac{1}{\left|S^{\prime}\right|} \sum_{s \in S^{\prime}} f_j(s) 
\end{equation}
The ratio measures how frequently the feature is activated within the subset $S^{\prime}$ relative to the total number of samples in the subset. At this point, we can define the stability and discriminability of features.

\begin{myDef} 
\textbf{Stable Feature}: A feature $f_j$ is defined as stable if, for any sufficiently large subset of samples $S^{\prime} \subseteq S$, the active ratio $r\left(f_j, S^{\prime}\right)$ remains within an $\epsilon$-bound of the overall active ratio $r\left(f_j, S\right)$ across the entire sample set, regardless of variations in sample size or composition. Formally, $f_j$ is stable if:
\begin{equation}
\forall S^{\prime} \subseteq S,\left|S^{\prime}\right| \geq n_0, \quad\left|r\left(f_j, S^{\prime}\right)-r\left(f_j, S\right)\right| \leq \epsilon    
\end{equation}
where $\epsilon>0$ is a small constant, and $n_0$ represents a minimum threshold for the size of $S^{\prime}$ to ensure the stability condition holds.
\end{myDef}

When we consider discriminability, there is a need to focus on the category to which the sample belongs. Thus, let $C=\left\{C_1, C_2, \ldots, C_k\right\}$ be a set of $k$ classes, and $S_k \subseteq S$ be the subset of samples belonging to class $C_k$. The active ratio of feature $f_j$ in class $C_k$ is given by:
\begin{equation}
  r\left(f_j, S_k\right)=\frac{1}{\left|S_k\right|} \sum_{s \in S_k} f_j(s)  
\end{equation}

\begin{myDef}
\textbf{Discriminative Feature}: A feature $f_j$ is discriminative if its active ratio differs significantly between at least two classes, $C_p$ and $C_q$. Specifically, there exists a threshold $\delta > 0$ such that:
\begin{equation}
  \exists C_p, C_q \in C, p \neq q, \quad\left|r\left(f_j, S_p\right)-r\left(f_j, S_q\right)\right| \geq \delta  
\end{equation}
\end{myDef}
Furthermore, the discriminative nature of the feature should be independent of the relative class sizes, meaning that the difference in activation should remain consistent despite variations in the proportion of samples in different classes. Mathematically, for any subset $\tilde{S}_p \subseteq S_p$ and $\tilde{S}_q \subseteq S_q$, where $\left|\tilde{S}_p\right| \neq\left|S_p\right|$ or $\left|\tilde{S}_q\right| \neq\left|S_q\right|$, the discriminative property still holds:
\begin{equation}
    \left|r\left(f_j, \tilde{S}_p\right)-r\left(f_j, \tilde{S}_q\right)\right| \geq \delta
\end{equation}

% \begin{figure}
%     \centering
%     % \setlength{\abovecaptionskip}{0.5cm}
%     \includegraphics[width=\linewidth]{Figure/feature_diff_10.pdf}
%     \caption{Discriminative change of Top 10 discriminative features in the training set during the test phase}
%     \label{fig:f1_family}
% \end{figure}
\begin{figure*}[htbp]
    \centering
    \begin{subfigure}[t]{0.48\textwidth}  
        \centering
        \includegraphics[width=1.0\textwidth]{Figure/feature_diff_10.pdf}
        \caption{}
        \label{fig:diff}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{Figure/feature_importance_10.pdf}
        \caption{}
        \label{fig:importance}
    \end{subfigure}
    
    \caption{(a) and (b) illustrate changes in the Discriminability of the top 10 discriminative training features and the top 10 important testing features, respectively. ``Discriminability'' is defined as the absolute difference in active ratios between benign and malicious samples. The grey dotted line indicates the start of the testing phase, with preceding values representing each feature's discriminability across months in the training set.}
    \label{fig:feature_discrimination}
\end{figure*}


\subsubsection{Failure Due to Learning Unstable Discriminative Features}
\label{motivation: failure}
The high test set performance of the malware detector within the same period suggests that it effectively learns discriminative features to distinguish benign software from malware. However, our analysis reveals that performance degradation over time is mainly due to the model's inability to capture stable discriminative features from the training set. To illustrate this, we sample 110,723 benign and 20,790 malware applications from the Androzoo\footnote{https://androzoo.uni.lu} platform (2014-2021). Applications are sorted by release date, with 2014 samples used for training and subsequent data divided into 30 equally spaced test intervals. We extract DREBIN~\cite{Arpdrebin} features, covering nine behavioral categories such as hardware components, permissions, and restrict API calls, and select the top 10 discriminative features based on active ratio differences to track over time.

The model configuration follows DeepDrebin~\cite{Grossedeepdrebin}, a three-layer fully connected neural network with 200 neurons per layer. We evaluate performance in each interval using macro-F1 scores. As shown in Figure~\ref{fig:feature_discrimination}, although the top 10 discriminative features maintain stable active ratios, the detector’s performance consistently declines. We further examine feature importance over time using Integrated Gradients (IG) with added binary noise, averaging results across five runs to ensure robustness, as recommended by Warnecke et al.~\cite{IG_explain}.

Figure~\ref{fig:feature_discrimination} presents the top 10 discriminative (a) and important features (b) identified by the model and their active ratio changes. While stable, highly discriminative features from the training set persist through the test phase, the ERM-based detector often relied on unstable features whose discriminative power fluctuated over time. This reliance leads to inconsistent model performance, stabilizing only when the feature discriminative power remains steady. Thus, we attribute the failure of ERM-based malware detectors in drift scenarios to their over-reliance on these unstable features and under-learning of already existing stable discriminative features, limiting its generalization to new samples.

% Figure.\ref{fig:importance} presents the top 10 important features identified by the model and their active ratio changes. The results show that while the highly discriminative features in the training set remained relatively stable during the test phase, the detector trained under empirical risk minimization (ERM) tended to rely on transient discriminative features. The discriminative power of certain features that the model focused on significantly fluctuated during the test phase, and does not seem to be significant enough in the training set. Moreover, when the discriminative power of features remained stable, the model’s performance also stabilized. Therefore, we attribute the failure of ERM-based malware detectors in drift scenarios to their over-reliance on these unstable features and under-learning of already existing stable discriminative features, limiting its generalization to new samples.

Moreover, we observe that highly discriminative features are often associated with high-permission operations and indicate potential malicious activity. For instance, features like \verb|api_calls::java/lang/Runtime;->exec| and \verb|GET_TASKS| are rarely used in legitimate applications. This aligns with malware invariance over time, where core malicious intents remain stable even as implementation details evolve.

\begin{center}
\fcolorbox{black}{gray!10}{\parbox{.9\linewidth}{\textit{\textbf{Take Away}: There are stable and highly discriminative features representing invariance in the training samples, yet current malware detectors fail to learn these features leading to decaying models' performance.}}}
\end{center}


\subsection{Create Model to Learn Invariance}
\label{learn_invariant_feature}
Our discussion highlights the importance of learning stable, discriminative features for drift-robust malware detection. ERM captures features correlated with the target variable, including both stable and unstable information~\cite{understanding}. When unstable information is highly correlated with the target, the model tends to rely on it. Thus, the key challenge is to isolate and enhance stable features, aligning with the goals of invariant learning outlined in Section~\ref{invariant_learning}.
% Our preceding discussion emphasized the importance of learning stable discriminative features for building drift-robust malware detectors. The goal of Empirical Risk Minimization (ERM) is to capture features closely related to the target variable, including both stable and unstable information, and the model is more inclined to rely on transient information when it is more relevant to the target~\cite{understanding}. The main challenge is therefore to isolate the stable component, which is consistent with the invariant learning goal described in Section~\ref{invariant_learning}. 

However, applying invariant learning methods is challenging. Its effectiveness presupposes firstly that the environment segmentation can expose the unstable information that the model needs to forget~\cite{environment_label, env_label}. In malware detection, it is uncertain which application variants will trigger distribution changes. Effective invariant learning requires the encoder to produce rich and diverse representations that provide valuable information for the invariant predictor~\cite{yang2024invariant}. Without high-quality representations, invariant learning may fail. This is also reflected in Figure~\ref{fig:feature_discrimination}, where even in the training phase, the learnt features are still deficient in discriminating between goodware and malware, and hard to fully represent the execution purpose of malware, relying instead on easily confusing features.

Thus, given arbitrary malware detectors, our intuition is to use time-aware environment segmentation to naturally expose the instability in malware distribution drift. Within each environment, ERM assumptions guide associations with the target variable, while the encoder provides both stable and unstable features for the invariant predictor. By minimizing invariant risk, unstable elements are filtered, thereby enhancing the detector's generalization capability.

% Thus, given arbitrary malware detectors, our scheme aims to further extend the learning capability of the encoder to provide more learnable information to the invariant predictor by relying only on the time-aware environment segmentation. Minimizing the invariant risk, in turn, filters out instability in the feature representation, thus further enhancing the generalization ability of the malware detector.

\begin{center}
\fcolorbox{black}{gray!10}{\parbox{.9\linewidth}{\textit{\textbf{Take Away}: Invariant learning helps to learn temporal stable features, but it is necessary to ensure that the training set can expose unstable information and the encoder can learn rich and good representations.}}}
\end{center}




==> History/Review.tex <==
\section{Background}
In this section, we review the development of malware detectors robust to drift and the key components of invariant learning, laying the groundwork for proposing an temporal invariant representation learning solution tailored for Android malware detection.


% \subsection{Concept Drift Caused by Malware Evolution}
% \label{concept_drift_in_malware}
% Concept drift refers to the changes in the statistical properties of data over time, which can render models trained under the assumption of independent and identically distributed (i.i.d.) data ineffective. This causes new data distributions to gradually deviate from the original decision boundaries, significantly impairing malware detection performance. Researchers typically identify two main causes of concept drift in Android malware: 

% \begin{enumerate}
%     \item Technological evolution of malware: Even malware from the same family can evolve due to market updates, framework iterations, and new obfuscation techniques, altering the program architecture that implements the same semantics~\cite{malware_evolution_obf}. These changes lead to a shift in the feature distribution, causing the classification boundaries established by the original detectors to gradually become obsolete~\cite{malware_evolution_update}.
%     \item Emergence of unknown malware families: Learning-based classification models are generally trained on datasets with fixed categories. However, the emergence of new malware families and changes in trends can introduce previously unseen malware families during model inference~\cite{new_family}. These samples may not resemble any known malware from the training dataset, leading to unreliable confidence scores and incorrect classifications.
% \end{enumerate}

\subsection{Drift-robust Malware Detectors}
Existing approaches to enhancing model robustness against drift focus primarily on refining feature representations. One line of work aims to identify features that remain robust to distribution changes, either through manual or automated feature engineering, allowing models to learn patterns less influenced by malware evolution~\cite{apigraph}. Another approach anticipates potential future distribution patterns by employing specific training strategies. Lu~et al.~\cite{DOMR} constructs pseudo-unknown families in the training set and uses episode learning to help the model learn robust representations that can generalize to open environments. Episode-based training strategy is introduced in the few-shot learning that divides the training process into a large number of episodes~\cite{episode_learning_1, episode_learning_2}, each simulating a task with limited samples, to foster representation learning. Here, the unknown families are treated as low-sample tasks. This method primarily addresses drift caused by the emergence of new families and requires managing an excessive number of episodes due to the need to cover all families in the training set. Yang et al.~\cite{scrr} propose the use of feature de-entanglement to keep the features as independent as possible during the model training process, minimizing their spurious correlations to preserve invariant information. However, the correlation between malware features is often critical, as certain sensitive API calls or intent combinations may be directly indicative of malicious behavior, and simply reducing feature correlation may be suboptimal. Angioni~et al.~\cite{svm_ce} introduce a feature stability metric for linear classifiers in the Drebin feature space, contributing insights for drift robustness in linear models but with limited applicability to complex feature relationships and non-linear models.

These prior methods seek to enhance invariant feature information by mitigating instabilities, which aligns with our approach. However, due to the diverse evolution and complexity of malware, pinpointing the precise cause of drift remains challenging. Strategies that rely on assumptions, such as drift being driven by new malware families, are limited. Instead, recognizing that distribution drift inevitably occurs over time motivates our exploration of temporally invariant information.

\subsection{Invariant Learning}
\label{invariant_learning}
\subsubsection{Notations}
Assume that the training data $\mathcal{D}_{tr}$ is collected from multiple environments $e \in \mathcal{E}$, i.e., $\mathcal{D}_{tr}=\{D^e_{tr}\}_{e \in \mathcal{E}}$. Let the input space be $x \in \mathcal{X}$ and the target space be $y \in \mathcal{Y}$, and for the sample observations from each environment denoted $x,y \sim p(x,y|e)$, the samples within the environments obey an independent and identical distribution. Suppose a classification model $\mathcal{M}$, denoted as a composite function $\mathcal{M}=c \circ \phi$. where $\phi:\mathcal{X} \rightarrow \mathcal{H}$ denotes a feature encoder that maps the input samples into a feature representation space $\mathcal{H}$, and $\phi(x) \in \mathcal{H}$ is the ``representation'' of sample $x$. The $c:\mathcal{H} \rightarrow \mathcal{Y}$ denotes a classifier that maps the feature representation to the logits space of $\mathcal{Y}$. 


\subsubsection{Learning Invariant Representation}
In test environments where distribution drift exists, the test data $\mathcal{D}_{ts}$ may come from a distribution $p(x,y|e_{ts})$ that does not appear in the training set, i.e. $e_{ts} \notin \mathcal{E}$. Robustness to drift yields lower error rates on unknown test data distributions.

Invariant learning enhances the generalization ability of a model to unknown distributions by learning label distributions that are invariant across training environments. Its goal is to develop a classifier $c(\cdot)$ that satisfies the environmental invariance constraint (EIC)~\cite{EIC}:

\begin{equation}
\mathbb{E}\left[y \mid \phi(x), e\right] = \mathbb{E}\left[y \mid \phi(x), e^{\prime}\right], \quad \forall e, e^{\prime} \in \mathcal{E},
\end{equation}

where $e$ and $e'$ denote different environments to which the samples belong. This constraint is integrated into the training objective through a penalty term. Thus, the goal can be formalized as:

\begin{equation}
\min _f\sum_{e \in \mathcal{E}} R^e_{erm}(f)+\lambda \cdot \operatorname{penalty}\left(\left\{S^e(f)\right\}_{e \in \mathcal{E}}\right),
\end{equation}

where $R^e_{erm}(f) = \mathbb{E}_{p(x,y|e)}[\ell(f(x),y)]$ represents the expected loss on environment $e$. Empirical risk minimization (ERM) is to minimize this expected loss within each environment. $S^e(f)$ is some statistic of the model in $e$ (see next), and the penalty is to constrain the change in this statistic to control the degree of deviation from the EIC. Optimizing this objective prevents mapping all $x$ to the same value to satisfy environmental invariance, as it encourages the predictive utility of $\phi$ by minimizing expected loss. In addition, the form of the penalty term is variable to achieve constraints for different objectives. Krueger et al.~\cite{v-rex} proposed V-Rex such that $S^e(f)=R^e_{erm}(f)$, to minimize the variance of $S^e(f)$ in different environments. In CLOvE~\cite{causal_ir}, the penalty is defined as the sum of the calibration errors of the model in each environment. One widely used scheme is Invariant Risk Minimization (IRM) and its practical variant IRMv1 proposed by Arjovsky et al.~\cite{IRM_training}. The penalty term is the sum of $S^e(f)=\left\|\nabla_w R^e_{erm}(w \circ \phi)\right\|^2$. $w$ is a constant scalar multiplier of 1.0 for each output dimension, forcing the shared classifier to be optimal in all environments. 

\subsubsection{Split Environments for Invariant Learning}
Invariant learning relies on the premise that environments should be segmented to maximize inter-environment differences~\cite{IR_intro}. Earlier solutions where environment labels are known a prior knowledge~\cite{bottleneck_ir, empirical_ir}. However, in practice, such a clear and accurate environment index of the environment is always unavailable~\cite{environment_label,inaccessible_label_2}. Nowadays, solutions turn to studying invariant learning without environment labels. Creager et al.~\cite{EIC} propose environment inference for invariant learning (EIIL), where the environment labels of the training data are estimated employing prior clustering, after which invariant learning is performed. Teney et al.~\cite{unshuffling} explore environment segmentation in visual question-answering, using two approaches: one based on provided question-type labels, and another using unsupervised clustering to create environments. Their results indicate that natural segmentation outperforms unsupervised clustering. Regardless of whether environment segmentation is learned through additional optimization or based on dataset-provided information, it aims to expose and ignore unstable information across environments~\cite{IR_intro}. 

==> History_dlsp/Introduction.tex <==
\section{Introduction}
The rapid growth of Android applications has significantly increased the security risks posed by malware, which threatens user privacy, financial security, and sensitive data. Over the past decade, researchers have developed various Android malware detection techniques, yet these traditional methods continue to face fundamental challenges in real-world settings. The open and dynamic nature of the Android ecosystem makes detecting evolving malware difficult~\cite{transcend, transcending}. Moreover, the overreliance on specific datasets introduces biases in training, such as ambiguously timestamped data and randomly selected samples~\cite{tesseract}, which can degrade model reliability. Another major limitation of conventional detectors is their lack of explainability—most tools provide only feature importance scores rather than offering a clear, human-readable interpretation of malicious behaviors.

Large Language Models (LLMs) offer a promising paradigm shift in malware detection, differing fundamentally from conventional detectors. They realize zero-shot inference relying on vast pre-trained knowledge instead of specifically labelled datasets~\cite{large_zero,toolformer}, allowing them to handle the evolving malware and potential training bias. Furthermore, existing malware detection tools that incorporate explainability techniques for deep neural networks typically focus on feature-level importance analysis instead of offering meaningful interpretations of malicious behaviors and Indicators of Compromise (IoCs). The advanced generative capabilities of LLMs present an opportunity to bridge this gap by providing human-readable comprehension, thereby enhancing malware analysis from both an accuracy and interpretability perspective.


However, despite their potential, LLMs are not omnipotent, particularly when applied to Android malware, which is characterized by complex function invocations, multi-component structures, and obfuscation techniques. Three key challenges hinder the effectiveness of LLMs: (1) \textit{\textbf{Limited LLM context window}}: Android malware usually contains thousands of classes to realize different functionalities. Directly feeding their decompiled code is infeasible, because none of the current LLMs can handle such large context window demands. Simply truncating the input leads to the loss of context information. (2) \textit{\textbf{Complex program structures}}: Unlike natural language, code follows a non-sequential structure with deeply nested dependencies across classes and intricate API interactions, especially in Android applications. This structural complexity makes it challenging for LLMs, which primarily rely on token sequences, to understand malicious behavior accurately. (3) \textit{\textbf{Sparse malicious behaviors}}: While Android malware executes unauthorized actions, it must also maintain benign functionalities to operate seamlessly across different devices. It submerges malicious patterns in normal calls which is hard to detect. At its core, these challenges highlight a fundamental requirement: 
\begin{center}
\fcolorbox{white}{gray!10}{\parbox{.9\linewidth}{\textit{Can we extract crucial structural and semantic information from complete application to guide LLMs in detecting Android malware?}}}
\end{center}
The process by which human analysts analyze malicious software in the real world follows this requirement. They identify suspicious APIs, interfaces, and function calls, analyzing their contextual relationships to detect malicious behavior within extensive application code. Our framework aims to guide LLMs in replicating this analytical process, enhancing automated Android malware detection and reasoning.

To tackle these difficulties and fulfil the demands, we propose LAMD, a novel and practical framework that enables LLMs to detect and reason about Android malware. LAMD consists of two core components: key context extraction and tier-wise code reasoning. Specifically, we analyse APK files statically and use our designed backward slicing algorithm to extract suspicious variables, instructions, and invocations indicating potentially malicious context. This process ensures that only relevant program structures are fed into the LLM, minimizing interference from unrelated functionalities. Additionally, we introduce a tier-wise reasoning mechanism coupled with factual consistency verification to ensure the reliability of summary transfer between tiers. This work lays the foundation for future research on exploring the reasoning capabilities of LLMs for detecting complex malware like Android malware in dynamic threat landscapes. The main contributions of this paper are as follows:

\begin{itemize}
    \item We propose the first LLM-powered practical Android malware detection framework, LAMD, which unlocks LLMs' ability for complex malware detection and reasoning in dynamic scenarios, providing heuristics for LLM-enhanced malware-related tasks.
    \item We enhance LAMD with a key context extractor and tier-wise code reasoning to filter out unrelated functionalities and capture semantics across API-to-function and function-to-function relationships. A targeted factual consistency verification strategy ensures intermediate correctness from the start of the tier-wise reasoning process.
    \item We evaluate LAMD on a constructed dataset\footnote{The dataset and code repository will be open-source for further research on LLM-based malware tasks.} that reflects the real-world setting and confirms the efficiency of LAMD in detecting and reasoning Android malware compared with commonly used detectors. 
\end{itemize}



% extracting essential structural and semantic information from APKs to effectively guide LLMs in identifying potentially malicious behaviors.




% Furthermore, the advanced generation and comprehension capabilities of LLM provide an opportunity to bridge the gap between feature-level explanations for malware detection and human-readable understanding.

% Furthermore, there is still a gap between feature-level explanations and human-readable comprehension for malware detection. The advanced generative capabilities of LLMs present an opportunity to offer understandable\ interpretations of malicious behaviors 


==> History_dlsp/Methodology.tex <==
\section{Methodology}
This section outlines the core components of our framework, LAMD, and how they cooperate to detect and understand Android malware efficiently.

\subsection{Overall Architecture}
The primary objective of LAMD is to extract essential functionalities and their contextual information, which are then fed into LLMs to generate both detection and reasoning results. The framework consists of two key components: (1) Key Context Extraction and (2) Tier-Wise Code Reasoning, detailed as follows:
\begin{itemize}
    \item \textbf{Key Context Extraction}: This component first identifies suspicious APIs, using them as seed points for context extraction. It then analyzes the control and data dependencies associated with these APIs within the target application. By leveraging this information, we construct a set of call relationships that encapsulate potentially malicious contexts, providing a structured representation of critical interactions.
    \item \textbf{Tier-wise Code Reasoning}: To maintain contextual relationships while managing context length, we adopt a tier-wise reasoning approach for malware detection. Three tiers correspond to functions, APIs and the APK respectively. The output of each tier is served as the input to the next one. Factual consistency is verified after each first-tier analysis to mitigate error propagation from the source.
\end{itemize}
Figure shows the pipeline of our framework. Overall, the raw input to LAMD is the application files, after which the suspicious APIs and their sliced contexts are extracted as the input to LLMs. Then the malicious behavior of the application is determined by two tiers of code reasoning.

\subsection{Key Context Extraction}
\subsubsection{Suspicious API Collection}
Malware exploits system vulnerabilities or API permissions to steal data, manipulate resources, or maintain persistence. Many attacks rely on API calls indicative of malicious behavior. We perform static analysis on APKs to extract suspicious API calls as key context to identify malware. Let $\mathcal{A} = \{a_1, a_2, \ldots, a_n\}$ be the set of all API calls in an APK. A subset $\mathcal{A}_{sus} \subset \mathcal{A}$ is deemed suspicious if it interacts with sensitive components, executes malware-associated operations or exposes sensitive data. These APIs fall into two categories:
\begin{itemize}
    \item \textit{Sensitive data access APIs}: While many apps handle sensitive data, assessing developer trustworthiness is challenging. Smartphone OSs implement permission-based access control, requiring declared permissions in the APK manifest for APIs enforcing permission checks. Additionally, Some APIs, like \verb|getPrimaryClip()| (clipboard access), bypass permission enforcement. We consider these two scenarios and classify an API $a_i$ is in this category because (1) requires permissions for access control or (2) directly provides access to sensitive user data without requiring permissions.
    \item \textit{Sensitive data transmission APIs}: It is also crucial to monitor potential channels through which sensitive information may leak to an adversary. Malicious applications often exploit these APIs to exfiltrate data to external services, commonly referred to as sink APIs. an API call $a_j$ is classified as sensitive if it attends to transfer sensitive data to external environments.
\end{itemize}

To extract suspicious APIs, we leverage publicly available knowledge based on PScout~\cite{pscout}, SuSi~\cite{susi} and Flowdroid~\cite{flowdroid} to label them. In the real-world setting, not every application contains suspicious APIs, these samples should be treated individually, which is acceptable, as traditional learning-based malware detectors are also hard to handle.


\subsubsection{Backward Program Pruning}
While extracting suspicious APIs is helpful, analyzing them in isolation often fails to reveal their contextual behavior. For example, a messaging app legitimately uses \verb|sendTextMessage()|, while malware may exploit it to send premium-rate SMS without user consent. To capture behavioral intent, we extract functions invoking suspicious APIs and filter out unrelated parts. Specifically, for each API $a_i \in \mathcal{A}_{sus}$, we locate the calling function $f_i$, and construct its control flow graph(CFG), $G = <N, E>$, to prepare for analysis dependency relationships, where each node $n \in N$ is either a basic block or a single instruction, and edges $(e_1, e_2) \in E$ define control flow. CFGs can be large and may include irrelevant instructions. To refine them, we apply backward slicing, isolating only instructions affecting the suspicious API invocation. A slice $S$ is defined by a slicing criterion $C = <s, V>$ where $s$ is the statement invoking $a_i$ and $V$ includes all parameters. We classify relevant variables as: (1) \textit{Direct relevant variables}: Variables' values can affect variable $v \in V$ of $a_i$  (2) \textit{Indirect relevant variables}: Variables in branch statements whose value affects invocation of $a_i$. The backward slicing is to select the set of instructions in $\mathcal{P}$ that directly or indirectly affect the execution or parameters of $a_i$. The backward slicing algorithm consists of two steps to ensure completeness in complex branch structures:
\begin{itemize}
    \item \textbf{Variable retrieval}: Identify all variables contributing to the parameters (and internal states) used by the suspicious API and store them in a candidate set.
    \item \textbf{Slices extraction}: Append instructions related to variables collected in the first step.
\end{itemize}

After slicing, we generate sliced CFGs for each sensitive API, preserving essential control flow and statements. Notably, If undeclared variables remain in a sliced function, inter-procedural backward slicing is recursively applied to its callers until all variables are resolved. The details of slicing algorithm are shown in Appendix~\ref{slicing}

\subsection{Tier-wise Code Reasoning}
Having identified the suspicious APIs and their surrounding instructions, we adopt a two-stage summarization strategy to (a) mitigate the token-length constraints in Large Language Models (LLMs) and (b) analyze how APIs interrelate in producing potential malicious behavior. The detailed prompts used in this stage are shown in Appendix~\ref{prompt}

\subsubsection{Function Behavior Summarization}
Although we can simply feed each suspicious API to an LLM for summarization, malicious behaviors often emerge when multiple APIs work in combination. To reflect these interdependencies, we group suspicious APIs following their associations.

We define an API group $\mathcal{G}_k$ as a set of APIs that share at least one calling function or exhibit overlapping usage of variables. Formally, if $f(a_i)$ denotes the set of function where API $a_i$ is invoked, then $\mathcal{G}_k=\left\{a_i \in \mathcal{A}_{\text {sus }} \mid \exists a_j \in \mathcal{G}_k \text { such that } f\left(a_i\right) \cap f\left(a_j\right) \neq \emptyset\right\}$. Each group $\mathcal{G}_k$ therefore captures a cluster of suspicious APIs that might collectively escalate malicious actions. 

After grouping, each $\mathcal{G}_k$ and its associated sliced CFGs (from the backward slicing results) are fed into the LLM, prompting it to produce a high-level behavioral description. This helps LLM recognize the combined functionality to reveal the different semantics generated by the API's joint calls in the current application context. An intuitive example is that if the API \verb|getDeviceId()| and \verb|sendTextMessage()| are grouped, the app may be exfiltrating sensitive information via SMS. 

\subsubsection{Factual Consistency Checking}
Generating code or behavior summaries using LLMs carries the risk of hallucinations, where the model invents facts inconsistent with the actual instructions. We perform a consistency check on each function behaviour summary to mitigate error accumulation before moving to final APK-level detection.

Inspired by factual consistency verification~\cite{cloze, factasking}, we design a structured template to capture data dependencies in sliced CFGs. To enhance inference, we omit certain dependency details from textual descriptions and prompt the LLM to infer missing relationships. We define seven data dependencies in two categories: variable-to-API interactions (direct, transitive, conditional, and loop dependencies) and inter-variable relationships (parallel, derived, and control dependencies). The first category captures how variables affect API execution through assignment, call chains, control flow, or iteration. The second describes variable interactions, including joint computation, derivation, and control influence. Appendix~\ref{datadependency} shows details about these data dependencies and their descriptions.

To evaluate the reliability of generated summaries, we propose a Data Relation Coverage (DRC) metric:
\begin{equation}
DRC = \frac{\#\{\text{correctly completed dependencies}\}}{\#\{\text{all selected dependencies}\}}.
\end{equation}
If the LLM can accurately restore or infer a sufficient fraction of these omitted dependencies (i.e., $DRC \ge \theta$, where $\theta$ is a reliability threshold), we deem the function behavior summaries to be factually consistent.   Otherwise, it is revised or discarded to minimize inaccuracies.

\subsubsection{Application Maliciousness Reasoning}
In this stage, we collect all verified summaries from each API group $\mathcal{G}_k$ and feed them into the LLM again to produce a final holistic analysis. This process enables APK-level classification, where the LLM synthesizes group-level insights to determine whether the APK is benign or malicious, considering interactions between API groups that may amplify suspicious behavior. Additionally, the LLM generates Indicators of Compromise (IoCs), providing a concise explanation that highlights accessed sensitive data, external transmissions, and unusual control flow or permission requests, improving transparency and fostering user trust. 






==> History_dlsp/Methodology2.6.tex <==
\section{Methodology}
This section outlines the core components of our framework, LAMD, and how they cooperate to detect and understand Android malware efficiently.

\subsection{Overall Architecture}
The LAMD framework is designed to extract essential functionalities and their contextual information, enabling LLMs to generate both detection and reasoning results. It consists of two key components: (1) Key Context Extraction and (2) Tier-wise Code Reasoning, detailed as follows:
\begin{itemize}
    \item \textbf{Key Context Extraction}: This module identifies suspicious APIs as seed points and analyzes their control and data dependencies within the application. Constructing call relationships that encapsulate potentially malicious interactions, provides a structured representation of critical program behaviors.
    \item \textbf{Tier-wise Code Reasoning}: To preserve contextual integrity while managing token limitations, LAMD employs a tiered reasoning strategy. It processes information at three levels—function, API, and APK—where each tier’s output informs the next. To mitigate error propagation, factual consistency verification is applied at the first tier.
\end{itemize}
Figure~\ref{fig:arch} shows the pipeline of our framework. Overall, the raw input to LAMD is the APK files, after which the suspicious APIs and their sliced contexts are extracted as the input to LLMs. Then the malicious behavior of the application is determined by three tiers of code reasoning.

\subsection{Key Context Extraction}
\subsubsection{Suspicious API Collection}
Malware exploits system vulnerabilities or API permissions to steal data, manipulate resources, or maintain persistence. Many attacks rely on sensitive API calls to implement malicious behaviors. We perform static analysis on APKs to extract suspicious APIs as key context to identify malware. Let $\mathcal{A} = \{a_1, a_2, \ldots, a_n\}$ be the set of all API calls in an APK. A subset $\mathcal{A}_{sus} \subset \mathcal{A}$ is deemed suspicious if it interacts with sensitive components, executes malware-associated operations or exposes sensitive data. These APIs fall into two categories:
\begin{itemize}
    \item \textit{Sensitive data access APIs}: While many apps handle sensitive data, assessing developer trustworthiness is challenging. Smartphone OSs implement permission-based access control, requiring declared permissions in the APK manifest for APIs enforcing permission checks. Additionally, Some APIs, like \verb|getPrimaryClip()| (clipboard access), bypass permission enforcement. An API $a_i$ falls into this category if it either: (1) requires explicit permissions for access control, or (2) grants direct access to sensitive user data without permission enforcement.
    \item \textit{Sensitive data transmission APIs}: Monitoring potential data exfiltration channels is critical, as malware often exploits these APIs—commonly referred to as sink APIs—to transmit sensitive information to external entities. An API $a_j$ is classified as suspicious if it facilitates the transfer of sensitive data to an external environment.
\end{itemize}

To extract suspicious APIs, we leverage publicly available knowledge based on PScout~\cite{pscout}, SuSi~\cite{susi} and Flowdroid~\cite{flowdroid} to label them. In a real-world setting, not every application contains suspicious APIs. These samples should be treated individually, where traditional learning-based malware detectors also struggle to handle~\cite{he2022msdroid}.


\subsubsection{Backward Program Pruning}
While extracting suspicious APIs is helpful, analyzing them in isolation often fails to reveal their contextual behavior. For example, a messaging app legitimately uses \verb|sendTextMessage()|, while malware may exploit it to send premium-rate SMS without user consent. To capture behavioral intent, we extract functions invoking suspicious APIs and filter out unrelated parts. Specifically, for each API $a_i \in \mathcal{A}_{sus}$, we locate the calling function $f_i$, and construct its control flow graph (CFG), $G = <N, E>$, to prepare for analysis dependency relationships, where each node $n \in N$ is either a basic block or a single instruction, and edges $(e_1, e_2) \in E$ define control flow. CFGs can be large and may include irrelevant instructions. To refine them, we apply backward slicing, isolating only instructions affecting the suspicious API invocation. A slice $S$ is defined by a slicing criterion $C = <s, V>$ where $s$ is the statement invoking $a_i$ and $V$ includes all parameters. We classify relevant variables as: (1) \textit{Direct relevant variables}: Variables' values can affect variable $v \in V$ of $a_i$  (2) \textit{Indirect relevant variables}: Variables in branch statements whose value affects invocation of $a_i$. The backward slicing is to select the set of instructions in $\mathcal{P}$ that directly or indirectly affect the execution or parameters of $a_i$. The backward slicing algorithm consists of two steps to ensure completeness in complex branch structures:
\begin{itemize}
    \item \textbf{Variable retrieval}: Identify all variables contributing to the parameters (and internal states) used by the suspicious API and store them in a candidate set.
    \item \textbf{Slices extraction}: Append instructions related to variables collected in the first step.
\end{itemize}

After slicing, we generate sliced CFGs for each sensitive API, preserving essential control flow and statements. Notably, If undeclared variables remain in a sliced function, inter-procedural backward slicing is recursively applied to its callers until all variables are resolved. The details of slicing algorithm are shown in Appendix~\ref{slicing}.

\subsection{Tier-wise Code Reasoning}
After detecting suspicious APIs and surrounding instructions, we apply a three-tier summarization strategy, refining APK behavior analysis from fine- to coarse-grained levels. This hierarchical approach improves malicious component identification while addressing LLM token-length constraints through separable reasoning. 

% The detailed prompts used in each stage are provided in Appendix~\ref{prompt}.

\begin{tcolorbox}[title=Tier 1: Function Behavior Summarization Prompt, colback=gray!20, colframe=black, colbacktitle=black, coltitle=white, sharp corners, fontupper=\small, fontlower=\small, before upper=\raggedright, before lower=\raggedright]
You are a cybersecurity expert specializing in Android malware analysis. Analyze the provided control flow graph including instructions related to sensitive API calls in detail.

Control Flow Graph: $\{CFG\_content\}$
\end{tcolorbox}

\subsubsection{Tier 1: Function Behavior Summarization}
In the previous stage, several functions invoking suspicious APIs are extracted and sliced to maintain the related context. Each sliced CFG of the function is fed to LLM to capture low-level code patterns and functionalities. 



\subsubsection{Tier 2: API Intent Awareness}
The context of a specific API is typically determined by a series of functions. Beyond function invocation relationships, it is crucial to examine how inter-function associations influence the API's intent. Due to diverse contexts, an API may appear in multiple Function Call Graphs (FCGs), each reflecting a different intent. For instance, \verb|getDeviceId()| is benign when used solely for local logging but becomes malicious when invoked within \verb|sendImeiToServer()|, where it exfiltrates the IMEI to a remote server. Therefore, at this mid-tier, all functions associated with a suspicious API are structured into multiple FCGs to analyze its overall intent. Each node in an FCG is represented by the function summary generated in the previous step. 

\begin{tcolorbox}[title=Tier 2: API Intent Awareness Prompt, colback=gray!20, colframe=black, colbacktitle=black, coltitle=white, sharp corners, fontupper=\small, fontlower=\small, before upper=\raggedright, before lower=\raggedright]
You are a cybersecurity expert specializing in Android malware analysis. Analyze the main functionality and behavior of the provided sensitive API based on all the function call graphs and a summary of the behavior of each function.

API name: $\{API\ name\}$ \\
API type: $\{access/transfer\}$\\
for $i$-th Function Call Graph: \\
\makebox[2em]{} FCG: $\{FCG\_content\}$ \\
\makebox[2em]{} $\{function\_name\} \{function\_summary\}$ 
\end{tcolorbox}



\subsubsection{Tier 3: APK Maliciousness Judgement}
After extracting intents from suspicious APIs in an APK, LLMs assess its maliciousness and justify their decision. They also generate Indicators of Compromise (IoCs), summarizing sensitive data access, external transmissions, and anomalous control flow or permission requests, enhancing transparency and user trust.


\begin{tcolorbox}[title=Tier 3: APK Maliciousness Judgement Prompt, colback=gray!20, colframe=black, colbacktitle=black, coltitle=white, sharp corners, fontupper=\small, fontlower=\small, before upper=\raggedright, before lower=\raggedright]
You are a cybersecurity expert specializing in Android malware analysis. Determine whether the application is MALWARE or BENIGN, citing indicators of compromise, evidence, and malicious patterns if present. Give a final prediction and key findings of your analysis.

for $i$-th API: \\
\makebox[2em]{}API name: $\{API\ name\}$ \\
\makebox[2em]{}API type: $\{access/transfer\}$\\
\makebox[2em]{}API intent: $\{API\ summary\}$
\end{tcolorbox}

% After getting intents of suspicious APIs in the specific APK, LLMs can review them to identify whether the APK is malicious or not and provide users with the basis of the determination. 

\subsubsection{Factual Consistency Checking}
Generating behavior summaries with LLMs risks hallucinations~\cite{nature24hallucinations}, producing facts inconsistent with instructions. To prevent error accumulation, we verify function-level summaries before higher-tier reasoning, leveraging their limited dependencies and concise structure.

Building on factual consistency verification~\cite{cloze, factasking}, we design a structured template to capture data dependencies in sliced CFGs. To enhance inference, we prompt the LLM to select corresponding data relationships from the input function based on specific definitions. We define five dependencies: variable-to-API interactions (direct, transitive, conditional) and inter-variable relationships (parallel, derived). The former tracks how variables influence API execution via assignments, call chains, and control flow, while the latter captures joint computation and derivation. Loop dependencies are excluded, as Soot expands loops when converting binary code to IR (Appendix~\ref{app:dataset}). Appendix~\ref{app:dataset} details these dependencies. For consistency verification, we integrate an in-context learning-based prompt with function summarization, querying the LLM to extract dependencies in the format: $<dependencies\ type>:<variable\ names>$.


\begin{tcolorbox}[title=Factual Consistency Verification Prompt, colback=gray!20, colframe=black, colbacktitle=black, coltitle=white, sharp corners, fontupper=\small, fontlower=\small, before upper=\raggedright, before lower=\raggedright]
The provided control flow graph represents a slice of the function, identifying variable relationships for each statement leading to the final invocation statement that invokes $\{function\_name\}$. The output should follow the template: $\{template\}$

Control Flow Graph: $\{CFG\_content\}$ 

There are FIVE types of relationships: \\
1. Direct: Variables used directly as function parameters.\\
\textit{Example}: $invoke r1.method(r2) \rightarrow {r1, r2}$ \\
2. Transitive: Variables whose values flow through assignments but are not directly used in the invocation. \\
\textit{Example}: $r2 = r3.getValue()$; \\
$invoke r1.method(r2) \rightarrow {r3}$ \\
...
\end{tcolorbox}

To evaluate the reliability of generated summaries, we propose a Data Relationship Coverage (DRC) metric:
\begin{equation}
DRC = \frac{\#\{\text{correctly completed dependencies}\}}{\#\{\text{all selected dependencies}\}}.
\end{equation}

A summary is considered factually consistent if the LLM accurately reconstructs variable dependencies, i.e., $DRC \ge \theta$, where $\theta$ is a reliability threshold. Otherwise, the summary is revised to mitigate inaccuracies.

% \subsubsection{Application Maliciousness Reasoning}
% In this stage, we collect suspicious API summaries for each APK and feed them into the LLM to produce a final holistic analysis. This process enables APK-level classification, where the LLM synthesizes API-level insights to determine whether the APK is benign or malicious. Additionally, the LLM generates Indicators of Compromise (IoCs), providing a concise explanation that highlights accessed sensitive data, external transmissions, and unusual control flow or permission requests, improving transparency and fostering user trust. 







==> History_dlsp/Review.tex <==
\section{Related Work}
In this section, we review conventional Android malware detection approaches, highlighting their real-world limitations and challenges. Additionally, we discuss recent advancements in LLM-powered malware reasoning, positioning our work within this emerging research direction.

\subsection{Learning-based Android Malware Detection}
Android malware detection methods fall into two main categories: rule-based and learning-based approaches. Rule-based methods rely on manually crafted signatures, making them ineffective against obfuscation and zero-day malware~\cite{unraveling}. 
Learning-based methods use static or dynamic analysis to extract predefined features, enabling automated detection. Due to the high cost of dynamic analysis, most models rely on static feature extraction through reverse engineering~\cite{Arpdrebin, Grossedeepdrebin}. Despite advancements, these models struggle with concept drift, where evolving malware variants degrade performance in real-world deployments~\cite{transcend, transcending}. Current works try to mitigate it, some of them focus on exploring robust features~\cite{scrr,damo,svm_ce,apigraph} and others leverage continual learning~\cite{continuous, tesseract,malware_evolution_update} or active learning~\cite{droidevolver, online_mal} to let models adapt to new distribution. However, these methods either target to specific feature space or introduce high retraining overhead and the risk of label poisoning~\cite{recda, labelless}. An additional challenge is explainability, which is critical for security analysis. Existing methods primarily use feature attribution techniques, providing importance scores without generating human-readable behavioral analysis~\cite{finer, belaid}. Therefore, the need for explainable and adaptable detection mechanisms has motivated the exploration of LLM-based approaches, which leverage extensive external knowledge and reasoning capabilities to improve malware analysis~\cite{code_explain,code_explain_2}.


\subsection{LLM-powered Malware Reasoning}
Large Language Models (LLMs) have recently gained traction in security applications, including code analysis~\cite{code_sum}, vulnerability detection~\cite{llm4vuln,llm4vuln_bench}, and malware classification~\cite{llm_syscall}. Unlike traditional machine learning models, LLMs possess zero-shot inference capabilities, allowing them to generalize beyond predefined training data and feature spaces~\cite{large_zero,toolformer}. This adaptability has led researchers to explore LLMs for malware detection and explanation, demonstrating their potential effectiveness in security tasks. Most existing studies focus on relatively simple malware ecosystems, such as npm packages~\cite{npm_malware}, PowerShell scripts~\cite{raconteur}, Linux binaries~\cite{llm_syscall}, and JavaScript-based threats~\cite{tactics}. 

Limited efforts have focused on Android malware, primarily in explanation and detection. The former provides a label as guidance to let LLMs generate analysis~\cite{malware_exploring,malware_decisioncentric}. The latter integrates LLMs into malware detection tasks by leveraging their semantic understanding. For instance, some approaches use LLMs to summarize features extracted from existing datasets (e.g., Drebin) and convert them into embeddings for classification~\cite{apppoet}, while it still struggles with generalizability in dynamic environments. Additionally, due to Android’s complex structure and large codebase, existing approaches rely on predefined feature spaces instead of raw code analysis, limiting LLMs' ability to capture API interaction contexts, program dependencies, and functional intent. This limitation motivates us to explore a framework that enables LLMs to reason about Android malware by integrating structural and semantic context, allowing for more comprehensive detection and perception of malicious behaviors in real-world scenarios.


% However, due to the high structural complexity and extensive code length of Android applications, existing methods primarily rely on predefined feature spaces rather than analyzing raw code directly. This limitation prevents LLM from fully leveraging its inference capabilities for comprehensive Android malware detection and behavioral analysis due to underdeveloped dynamic API interactions, program dependencies, and functional intent. It motivates us to explore a framework that enables LLMs to reason about Android malware by incorporating structural and semantic context, allowing for a more comprehensive and interpretable analysis of malicious behaviors.
 

==> Tex/ExpSetting.tex <==
\section{Experiment Details}
\label{expSet}
Our experiments are conducted on an RTX A6000 GPU. For LLM-based reasoning, we utilize GPT-4o-mini~\cite{openai}, selected for its high efficiency, cost-effectiveness, and strong reasoning capabilities. The Data Relation Coverage (DRC) threshold $\theta$ is set to 0.95 to balance computational efficiency and accuracy.


% \subsection{Human-Verified Test Set}


% \subsection{Summary Evaluation}

